Sensitivity of Transitions in Internal Rotor Molecules to a Possible Variation of the Proton-to-Electron Mass Ratio

Recently, methanol was identified as a sensitive target system to probe variations of the proton-to-electron mass ratio $\mu$ [Jansen \emph{et al.} Phys. Rev. Lett. \textbf{106}, 100801 (2011)]. The high sensitivity of methanol originates from the interplay between overall rotation and hindered internal rotation of the molecule -- i.e. transitions that convert internal rotation energy into overall rotation energy, or vice versa, give rise to an enhancement of the sensitivity coefficient, $K_{\mu}$. As internal rotation is a common phenomenon in polyatomic molecules, it is likely that other molecules display similar or even larger effects. In this paper we generalize the concepts that form the foundation of the high sensitivity in methanol and use this to construct an approximate model which allows to estimate the sensitivities of transitions in internal rotor molecules with $C_{3v}$ symmetry, without performing a full calculation of energy levels. We find that a reliable estimate of transition sensitivities can be obtained from the three rotational constants ($A$, $B$, and $C$) and three torsional constants ($F$, $V_3$ and $\rho$). This model is verified by comparing obtained sensitivities for methanol, acetaldehyde, acetamide, methyl formate and acetic acid with a full analysis of the molecular Hamiltonian. From the molecules considered, methanol appears to be the most suitable candidate for laboratory and cosmological tests searching for a possible variation of $\mu$.

==> chemfig.tex <==
%  __________________________________________________________________
% |                                                                  |
% |                                                                  |
% |                           chemfig v1.0a                          |
% |                                                                  |
% |                        September 18, 2011                        |
% |                                                                  |
% |__________________________________________________________________|
%
% This is chemfig.tex, the code of the "chemfig" package.
%
% Maintainer: Christian Tellechea
% E-mail    : unbonpetit@gmail.com
%             Comments, bug reports and suggestions are welcome.
% Licence   : Released under the LaTeX Project Public License v1.3c or
%             later, see http://www.latex-project.org/lppl.txt
% Copyright : Christian Tellechea 2010-2011
%
% The "chemfig" package consists of the 8 following files:
%   chemfig.tex (this file)
%   chemfig.sty (the package file for LaTeX)
%   t-chemfig.tex (the package file for conTeXt)
%   README
%   chemfig_doc_en.tex, chemfig_doc_en.pdf (english manual)
%   chemfig_doc_fr.tex, chemfig_doc_fr.pdf (manual in french)
%
% --------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
% %     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% --------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% --------------------------------------------------------------------

% Sauvegarde tous les catcodes des caract\`eres sp\'eciaux sauf #
\begingroup
	\def\X#1{\catcode\number`#1=\number\catcode`#1\relax}
	\expandafter\xdef\csname CF@savedcatcode\endcsname{%
		\X\[\X\]\X\:\X\(\X\)\X\,\X\-\X\=\X\~\X\!\X\?\X\<\X\>\X\;\X\*\X\|\X\@%
	}
\endgroup

% Pour la dur\'ee de lecture du package, changer les catcodes :
\catcode`\[12 \catcode`\]12 \catcode`\:12 \catcode`\(12
\catcode`\)12 \catcode`\,12 \catcode`\-12 \catcode`\=12
\catcode`\~12 \catcode`\!12 \catcode`\?12 \catcode`\<12
\catcode`\>12 \catcode`\;12 \catcode`\*12 \catcode`\|12
\catcode`\@11 \catcode`\#6  \catcode`\ 10

\def\CF@def#1{%
	\ifdefined#1%
		\errmessage{Package chemfig Error: the macro \string#1\space is already defined. Please, email the author.}%
	\fi
	\def#1%
}

\CF@def\CF@ver         {1.0a}
\CF@def\CF@date        {2011/09/18}
\CF@def\CF@fr@date     {18 septembre 2011}
\CF@def\CF@en@date     {September 18, 2011}
\CF@def\CF@package@name{chemfig}

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\ifdefined\tikzpicture\else
		\def\CF@next@action{\input tikz.tex}%
		\expandafter\CF@next@action
	\fi
	\immediate\write\m@ne{Package: \CF@package@name\space\CF@date\space\space v\CF@ver\space\space Draw molecule with an easy syntax}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@firstofone#1{#1}
	\long\def\@gobble#1{}
	\long\def\@gobbletwo#1#2{}
	\def\@car#1#2\@nil{#1}
	\def\@makeother#1{\catcode`#1=12\relax}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
	\def\space{ }
	\CF@def\printatom#1{\ifmmode\rm#1\else$\rm#1$\fi}% \printatom pour TeX et ConTeXt
\else% fin des d\'efinitions LaTeX
	\CF@def\printatom#1{\ensuremath{\mathrm{#1}}}% \printatom pour LaTeX.
\fi

\newcount\CF@cnt@atomingroup
\newcount\CF@cnt@groupnumber
\newcount\CF@cnt@atomnumber
\newcount\CF@cnt@cycle

\newif\ifCF@incycle
\newif\ifCF@cyclearc
\newif\ifCF@definesubmol

\newdimen\CF@dim

\newbox\CF@lewis@box
\newbox\CF@box@boxa
\newbox\CF@box@boxb
\newbox\CF@stuff@box

\newwrite\CF@unused

\CF@def\CF@sanitize@catcode{%
	\@makeother\[\@makeother\]\@makeother\:\@makeother\(\@makeother\)%
	\@makeother\,\@makeother\-\@makeother\=\@makeother\~\@makeother\!%
	\@makeother\?\@makeother\<\@makeother\>\@makeother\;\@makeother\*%
	\@makeother\|\@makeother\#\@makeother\@%
}

\CF@def\CF@node@content{\expandafter\printatom\expandafter{\csname atom@\number\CF@cnt@atomnumber\endcsname\CF@node@strut}}

\CF@def\chemskipalign{%
	\ifx\CF@bond@outcontentsaved\@empty% sauf si un \chemskipalign a \'et\'e fait \`a l'atome pr\'ec\'edent
		\global\let\CF@bond@outcontentsaved\CF@bond@outcontent% sauvegarder l'atome d'o\`u vient la liaison
	\fi
	\let\CF@node@strut\@empty
}

\CF@def\CF@empty@node{{}}

\CF@def\CF@cycle@inraduiscoeff{0.75}% coeff multiplicateur du rayon des arcs dans les cycles

\CF@def\setcrambond#1#2#3{%
	\def\CF@cram@basewidth{#1}%
	\ifx\@empty#2\@empty\def\CF@cram@dashlength{1pt}\else\def\CF@cram@dashlength{#2}\fi
	\ifx\@empty#3\@empty\def\CF@cram@dashsep{2pt}\else\def\CF@cram@dashsep{#3}\fi}
\setcrambond{}{}{}

\CF@def\setatomsep{\def\CF@atom@sep}% espacement des atomes li\'es
\setatomsep{}

\CF@def\setbondoffset{\def\CF@bond@offset}% offset des liaisons
\setbondoffset{2pt}

\CF@def\setdoublesep{\def\CF@double@sep}
\setdoublesep{2pt}

\CF@def\definesubmol{\CF@definesubmoltrue\CF@def@submol}
\CF@def\redefinesubmol{\CF@definesubmolfalse\CF@def@submol}

\CF@def\CF@def@submol#1{%
	\begingroup
		\def\CF@tmp@str{#1}%
		\catcode`[\@ne\catcode`]\tw@
		\futurelet\CF@toks@a\CF@test@nxttok
}

\CF@def\CF@test@nxttok{%
		\if[\noexpand\CF@toks@a
			\expandafter\expandafter\expandafter\CF@grab@optalias\expandafter\expandafter\expandafter{\expandafter\CF@tmp@str\expandafter}%
		\else
			\CF@swap@fi
			\expandafter\endgroup
			\expandafter\CF@def@submol@i\expandafter{\CF@tmp@str}{}%
		\fi
}

\CF@def\CF@grab@optalias#1#2{%
	\endgroup
	\begingroup
	\everyeof{\@nil}\endlinechar\m@ne
	\expandafter\assign@tonil\expandafter\CF@tmp@str\scantokens{#2}%
	\CF@expand@second{\endgroup\CF@def@submol@i{#1}}\CF@tmp@str
}

\CF@def\CF@def@submol@i#1#2#3{% #1 nom, #2 = code si liaison arrive de droite , #3 = code si liaison arrive de gauche
	\ifcat\relax\expandafter\noexpand\@car#1\@nil% si #1 est une s\'equence de contr\^ole
		\expandafter\ifdefined\@car#1\@nil
			\ifCF@definesubmol
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: the macro \expandafter\string\@car#1\@nil\space is already defined, the previous definition is lost on input line \the\inputlineno.}%
			\fi
		\fi
		\ifx\@empty#2\@empty
			\expandafter\def\@car#1\@nil{\@empty#3}%
		\else
			\expandafter\def\@car#1\@nil{%
				\romannumeral
				\ifdim\CF@current@angle pt>90pt
					\ifdim\CF@current@angle pt<270pt
						\expandafter\expandafter\expandafter\@firstoftwo
					\else
						\expandafter\expandafter\expandafter\@secondoftwo
					\fi
				\else
					\expandafter\@secondoftwo
				\fi
				{\z@#2}{\z@#3}}%
		\fi
	\else
		\ifcsname CF@@#1\endcsname
			\ifCF@definesubmol
				\immediate\write\CF@unused{Package \CF@package@name\space Warning:the submol "#1" is already defined, the previous definition is lost on input line \the\inputlineno.}%
			\fi
		\fi
		\ifx\@empty#2\@empty
			\expandafter\def\csname CF@@#1\endcsname{\@empty#3}% "\@empty" car tout ça sera 1-d\'evelopp\'e lorsque rencontr\'ee
		\else
			\expandafter\def\csname CF@@#1\endcsname{%
				\romannumeral% donnera le d\'eveloppement souhait\'e en 1 coup
				\ifdim\CF@current@angle pt>90pt
					\ifdim\CF@current@angle pt<270pt
						\expandafter\expandafter\expandafter\@firstoftwo
					\else
						\expandafter\expandafter\expandafter\@secondoftwo
					\fi
				\else
					\expandafter\@secondoftwo
				\fi
				{\z@#2}{\z@#3}}%
		\fi
	\fi
}

\CF@def\CF@if@integer#1{%
	\begingroup
		\afterassignment\CF@after@integer
		\CF@cnt@cycle0#1\relax
}

\CF@def\CF@after@integer#1\relax{%
	\endgroup
	\ifx\@empty#1\@empty\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}

\CF@def\CF@swap@fi#1\fi{\fi#1}

\CF@def\CF@gobble@tonil#1\@nil{}

\CF@def\CF@expafterarg@ntimes#1#2#3{%
	\CF@expafterarg@ntimes@i{#1}{#3}%
	\expandafter\CF@swap@arg\expandafter{\CF@tmp@str}{#2}%
}

\CF@def\CF@expafterarg@ntimes@i#1#2{%
	\ifnum#1=\z@
		\def\CF@tmp@str{#2}%
	\else
		\CF@swap@fi
		\expandafter\CF@expafterarg@ntimes@i\expandafter{\number\numexpr#1-1\expandafter}\expandafter{#2}%
	\fi
}

\CF@def\CF@swap@arg#1#2{#2{#1}}

\CF@def\CF@expand@second#1#2{\expandafter\CF@swap@arg\expandafter{#2}{#1}}

\CF@def\CF@swap@char#1#2{#2#1}

\CF@def\CF@expand@afterfirst#1#2{\expandafter\CF@swap@char\expandafter{#2}{#1}}

\CF@def\CF@edef@second#1#2{%
	\edef\CF@tmp@str{#2}%
	\expandafter\CF@swap@char\expandafter{\CF@tmp@str}{#1}%
}

\CF@def\CF@add@tocs#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\CF@def\CF@expadd@tocs#1#2{\expandafter\CF@add@tocs\expandafter#1\expandafter{#2}}

\CF@def\CF@edefadd@tocs#1#2{%
	\edef\CF@tmp@str{#2}%
	\expandafter\CF@add@tocs\expandafter#1\expandafter{\CF@tmp@str}%
}

\CF@def\CF@if@firsttokmatch#1#2{% est ce que #1 et #2 commencent par les m\^emes tokens ?
	\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
	\futurelet\CF@toks@b\CF@gobble@tonil#2\relax\@nil
	\ifx\CF@toks@a\CF@toks@b\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}

\CF@def\CF@if@firsttokin#1{% teste si le token qui commence #1 appartient aux tokens mis dans #2
	\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
	\CF@if@firsttokin@i
}

\CF@def\CF@if@firsttokin@i#1{%
	\ifx\@empty#1\@empty
		\expandafter\@secondoftwo
	\else
		\futurelet\CF@toks@b\CF@gobble@tonil#1\relax\@nil
		\ifx\CF@toks@a\CF@toks@b
			\expandafter\expandafter\expandafter\@firstoftwo
		\else
			\CF@swap@fi\CF@swap@fi
			\expandafter\CF@if@firsttokin@i\expandafter{\@gobble#1}%
		\fi
	\fi
}

\CF@def\CF@if@instr#1#2{%
	\def\CF@if@instr@i##1#2##2\@nil{\ifx\@empty##2\@empty\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}%
	\CF@if@instr@i#1\@@nil#2\@nil
}

\CF@def\CF@after@space#1 #2\@nil{#2}

\CF@def\CF@seek@node#1#2#3{% cherche un noeud au d\'ebut de #1 l'assigne dans la sc #2 et met le reste dans #3
	\let#2\@empty
	\def#3{#1}%
	\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
	\ifx\CF@toks@a\@sptoken\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\expandafter\CF@seek@node@i\expandafter{\CF@after@space#1\@nil}#2#3}% ignore l'espace qui commence un groupe d'atome
		{\CF@seek@node@i{#1}#2#3}%
}

\CF@def\CF@seek@node@i#1#2#3{%
	\ifx\@empty#1\@empty
		\let#3\@empty
	\else
		\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
		\ifx\CF@toks@a\@sptoken\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\CF@add@tocs#2{ }%
			\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\CF@after@space#1\@nil}#2#3%
			}%
			{\ifx\CF@toks@a\bgroup\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
				{\CF@expadd@tocs#2{\expandafter{\@car#1\@nil}}%
				\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\@gobble#1}#2#3%
				}%
				{\CF@if@firsttokin@i{-=(*<>!~}%
					{\def#3{#1}}%
					{\CF@expadd@tocs#2{\@car#1\@nil}%
					\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\@gobble#1}#2#3%
					}%
				}%
			}%
	\fi
}

% on sait que #1 commence par -,=,~,<,>. On analyse cette liaison
% #2 reçoit le type de liaisons (1 pour -, 2 pour =, 3 pour ~)
\CF@def\CF@bond@findnum#1#2{%
	\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
	\edef#2{%
		\ifx-\CF@toks@a1%
		\else
			\ifx=\CF@toks@a2%
			\else
				\ifx~\CF@toks@a3%
				\else
					\ifx>\CF@toks@a4%
					\else
						\ifx<\CF@toks@a5%
						\else0% si 0 --> il y a une erreur non dûe \`a l'utilisateur
						\fi
					\fi
				\fi
			\fi
		\fi}%
	\ifnum#2>\thr@@% si c'est une liaison de Cram
		\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@gobble#1\@nil% chope le caract\`ere suivant
		\ifx:\CF@toks@a
			\edef#2{\number\numexpr#2+2}% si c 'est un ":", signe du pointill\'e, ajoute 2
		\else
			\ifx|\CF@toks@a
				\edef#2{\number\numexpr#2+4}% si c 'est un "|", signe du triangle \'evid\'e, ajouter 4
			\fi
		\fi
	\fi
}

\CF@def\CF@analyse@bondoffset#1,#2\@nil{%
	\def\CF@start@offset{#1}\def\CF@end@offset{#2}%
}

\expandafter\CF@def\expandafter\CF@grab@bondoffset\string#(#1)#2\@nil{%
	\ifx\@empty#1\@empty
	\else
		\CF@if@instr{#1},%
			{\CF@analyse@bondoffset#1\@nil}%
			{\def\CF@start@offset{#1}}%
	\fi
	\def\CF@remain@afterbond{#2}%
}

\CF@def\CF@analyse@bond#1#2{%
	\CF@bond@findnum{#1}#2%
	\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobble#1}%mange le premier signe de la liaison
	\let\CF@doublebond@type\z@
	\ifnum#2=\tw@% si c'est une double liaison, regarde s'il y a un + ou - derri\`ere
		\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@gobble#1\@nil
		\ifx^\CF@toks@a
			\let\CF@doublebond@type\@ne
			\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange le "^"
		\else
			\ifx_\CF@toks@a
				\let\CF@doublebond@type\tw@
				\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange le "_"
			\fi
		\fi
	\else
		\ifnum#2>5 % si c'est une laision de Cram pointill\'ee ou triangle \'evid\'e
			\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange un caract\`ere de plus
		\fi
	\fi
	\expandafter\expandafter\expandafter\CF@if@firsttokmatch\expandafter\expandafter\expandafter{\expandafter\CF@remain@afterbond\expandafter}\string##%
		{\expandafter\CF@grab@bondoffset\CF@remain@afterbond\@nil}%
		\relax
	\expandafter\expandafter\expandafter\CF@if@firsttokmatch\expandafter\expandafter\expandafter{\expandafter\CF@remain@afterbond\expandafter}\string @%
		{\expandafter\CF@grab@movearg\CF@remain@afterbond\@nil}%
		\relax
	\expandafter\CF@if@firsttokmatch\expandafter{\CF@remain@afterbond}[%
		{\expandafter\CF@analyse@optarg\CF@remain@afterbond\@nil\CF@remain@afterbond}%
		{\let\CF@current@stringangle\CF@default@stringangle
		\let\CF@current@length\CF@default@length
		\let\CF@current@fromatom\CF@default@fromatom
		\let\CF@current@toatom\CF@default@toatom
		\let\CF@current@tikz\CF@default@tikz
		\let\CF@movebond@name\@empty
		}%
	\ifCF@incycle
		\pgfmathparse{360/\CF@cycle@num+\CF@initcycle@angle}%
		\edef\CF@current@stringangle{::+\pgfmathresult}%
		\def\CF@initcycle@angle{0}%
		\let\CF@current@length\CF@default@length% et on ignore la longueur de liaison sp\'ecifi\'ee
	\fi
	\expandafter\CF@set@bondangle\expandafter{\CF@current@stringangle}\CF@current@angle
}

\CF@def\CF@set@bondangle#1#2{% le code de la direction est contenu dans #1, en sortie, #2 contient l'angle
	\ifx\@empty#1\@empty%
		\let#2\CF@default@angle
	\else
		\if:\expandafter\noexpand\@car#1\@nil
			\if:\expandafter\expandafter\expandafter\noexpand\expandafter\@car\@gobble#1\@nil
				\pgfmathparse{\CF@previous@angle+\expandafter\@gobble\@gobble#1}%
				\let#2\pgfmathresult
			\else
				\expandafter\def\expandafter#2\expandafter{\@gobble#1}
			\fi% puis normalise l'angle entre 0 et 360
			\ifdim\ifdim#2pt<\z@-\fi#2pt>360pt % si |#2|>360
				\pgfmathparse{#2-360*floor(#2/360)}%
				\ifdim\pgfmathresult pt<\z@\pgfmathparse{\pgfmathresult+360}\fi
				\let#2\pgfmathresult
			\else
				\ifdim#2pt<\z@
					\pgfmathparse{#2+360}%
					\let#2\pgfmathresult
				\fi
			\fi
		\else
			\ifnum#1>7
				\pgfmathparse{#1-floor(#1/8)*8}%
				\ifdim\pgfmathresult pt<\z@\pgfmathparse{\pgfmathresult+8}\fi
				\edef#2{\ifcase\expandafter\CF@int@part\pgfmathresult\@nil0\or45\or90\or135\or180\or225\or270\or315\else-1\fi}% angle =-1 --> erreur
			\else
				\edef#2{\ifcase#1 0\or45\or90\or135\or180\or225\or270\or315\else-1\fi}%
			\fi
		\fi
	\fi
}

\CF@def\CF@int@part#1.#2\@nil{#1 }

\CF@def\CF@analyse@movearg#1,#2\@nil#3{%
	\def#3{#1}\def\CF@movebond@coeff{#2}%
}

% Argument limit\'es l\'egitimes ici car #2 (qui est ce qui suit "@{<nom>}" dans l'argument optionnel) ne DOIT
% pas commencer par une accolade.
\expandafter\CF@def\expandafter\CF@grab@movearg\string @#1#2\@nil{%
	\CF@if@instr{#1},%
		{\CF@analyse@movearg#1\@nil\CF@movebond@name}%
		{\def\CF@movebond@name{#1}\def\CF@movebond@coeff{0.5}}%
	\def\CF@remain@optarg{#2}%
}

\CF@def\CF@testempty@andassign#1#2#3{\ifx\@empty#2\@empty\let#1#3\else\def#1{#2}\fi}

\CF@def\CF@sanitize@lastitem#1,\@empty#2\@nil{#1}

\CF@def\CF@parse@optlist#1,#2,#3,#4,#5\@nil{%
	\CF@testempty@andassign\CF@current@stringangle{#1}\CF@default@stringangle
	\CF@testempty@andassign\CF@current@length{#2}\CF@default@length
	\CF@testempty@andassign\CF@current@fromatom{#3}\CF@default@fromatom
	\CF@testempty@andassign\CF@current@toatom{#4}\CF@default@toatom
	\expandafter\CF@testempty@andassign\expandafter\CF@current@tikz\expandafter{\CF@sanitize@lastitem#5,\@empty\@nil}\CF@default@tikz
}%

\CF@def\CF@analyse@optarg[#1]#2\@nil#3{%
	\ifx\@empty#1\@empty
	\else
		\CF@expand@afterfirst{\CF@if@firsttokmatch{#1}}{\string @}%
			{\CF@grab@movearg#1\@nil}%
			{\let\CF@movebond@name\@empty
			\def\CF@remain@optarg{#1}}%
		\expandafter\CF@parse@optlist\CF@remain@optarg,\@empty,\@empty,\@empty,\@empty\@nil
		\def#3{#2}%
	\fi
}

\CF@def\CF@seek@submol{%
	\expandafter\CF@if@firsttokmatch\expandafter{\CF@remain@molecule}!%
		{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter
			\CF@remain@molecule\expandafter\expandafter\expandafter{\expandafter\@gobble\CF@remain@molecule}% enl\`eve le ``!''
		\ifcat\relax\expandafter\expandafter\expandafter\noexpand\expandafter\@car\CF@remain@molecule\@nil
			\CF@expafterarg@ntimes5{\def\CF@insert@submol}{\expandafter\@car\CF@remain@molecule\@nil}%
		\else
			\CF@expafterarg@ntimes3{\def\CF@insert@submol}{\csname CF@@\expandafter\@car\CF@remain@molecule\@nil\endcsname}%
		\fi
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@remain@molecule\expandafter\expandafter\expandafter
			{\csname CF@insert@submol\expandafter\expandafter\expandafter\endcsname\csname @gobble\expandafter\endcsname\CF@remain@molecule}%
		\CF@seek@submol
		}%
		\relax
}

\CF@def\CF@insert@emptygroup#1{% ins\`ere {} au d\'ebut de la sc #1
	\expandafter\def\expandafter#1\expandafter{\expandafter{\expandafter}#1}%
}

\CF@def\chemfig{\@testopt\CF@chemfig@i{}}

\CF@def\CF@chemfig@i[#1]{\@testopt{\CF@chemfig@ii[#1]}{}}

\CF@def\CF@chemfig@ii[#1][#2]{%
	\edef\CF@tmp@str{[remember picture,every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@\ifx\@empty#2\@empty\else,#2\fi},baseline\ifx\@empty#1\@empty\else,#1\fi]}%
	\expandafter\tikzpicture\CF@tmp@str
	\begingroup
		\let\CF@hook@list\@empty
		\ifx\CF@atom@sep\@empty\def\CF@atom@sep{3em}\fi
		\ifx\CF@cram@basewidth\@empty\def\CF@cram@basewidth{1.5ex}\fi
		\CF@incyclefalse
		\CF@cnt@groupnumber\z@
		\let\CF@last@action\z@% 0=d\'ebut du dessin 1=trac\'e d'un noeud 2=trac\'e d'une liaison
		\let\CF@start@offset\@empty
		\let\CF@end@offset\@empty
		\let\CF@bond@outcontentsaved\@empty
		\def\CF@cycle@anglecorrection{180/\CF@cycle@num}%
		\def\CF@default@angle{0}%
		\def\CF@default@stringangle{:0}% angle pris par d\'efaut si le champ est vide
		\def\CF@default@length{1}%
		\let\CF@default@fromatom\@empty% numero de l'atome d'o\`u partent les liaisons par d\'efaut
		\let\CF@default@toatom\@empty% num\'ero de l'atome o\`u arrivent les laisons par d\'efaut
		\let\CF@default@tikz\@empty
		\everyeof{\@nil}\endlinechar\m@ne
		\CF@sanitize@catcode
		\CF@chemfig@iii
}

\CF@def\CF@chemfig@iii#1{%
	\expandafter\assign@tonil\expandafter\CF@remain@molecule\scantokens{#1}%
	\expandafter\CF@chemfig@iv\expandafter{\CF@remain@molecule}%
	\endtikzpicture
	\let\CF@split@state\z@
}

\CF@def\CF@chemfig@iv#1{% #1 est le code de la mol\'ecule
	\ifnum\CF@last@action=\thr@@
		\ifCF@incycle
			\def\CF@default@angle{0}%
		\else
			\ifnum\CF@cnt@cycle=\z@% si c'est le d\'ebut d'un cycle
				\pgfmathparse{\CF@previous@angle+180+\CF@cycle@anglecorrection}% on met la liaison \`a +180° + correction
			\else
				\pgfmathparse{\CF@previous@angle-90+180/\CF@cycle@num}% sinon \`a la bissectrice du sommet du cycle
			\fi
			\let\CF@default@angle\pgfmathresult
		\fi
		\let\CF@default@stringangle\@empty
	\fi
	\let\CF@current@angle\CF@default@angle
	\def\CF@remain@molecule{#1}%
	\CF@seek@submol% alias en premier ?
	\if[\expandafter\expandafter\expandafter\noexpand\expandafter\@car\CF@remain@molecule\@nil
		\expandafter\CF@analyse@optarg\CF@remain@molecule\@nil\CF@remain@molecule
		\expandafter\CF@set@bondangle\expandafter{\CF@current@stringangle}\CF@current@angle
		\let\CF@default@angle\CF@current@angle
		\let\CF@previous@angle\CF@current@angle
		\unless\ifx\@empty\CF@current@stringangle\let\CF@default@angle\CF@current@angle\fi
		\unless\ifx\@empty\CF@current@length\let\CF@default@length\CF@current@length\fi
		\unless\ifx\@empty\CF@current@fromatom\let\CF@default@fromatom\CF@current@fromatom\fi
		\unless\ifx\@empty\CF@current@toatom\let\CF@default@toatom\CF@current@toatom\fi
		\unless\ifx\@empty\CF@current@tikz\let\CF@default@tikz\CF@current@tikz\fi
		\CF@seek@submol
	\fi
	\ifCF@incycle% si on commence un cycle
		\let\CF@current@angle\CF@previous@angle
	\else
		\let\CF@current@angle\CF@default@angle
	\fi
	\edef\CF@default@stringangle{:\CF@default@angle}%
	\let\CF@current@length\CF@default@length
	\let\CF@current@fromatom\CF@default@fromatom
	\let\CF@current@toatom\CF@default@toatom
	\let\CF@current@tikz\CF@default@tikz
	\ifnum\CF@last@action=\z@
		\let\CF@previous@angle\CF@default@angle
		\node(CF@node){};
		\expandafter\CF@if@firsttokin\expandafter{\CF@remain@molecule}{-=(*~?<>}%
			{\CF@insert@emptygroup\CF@remain@molecule}%
			\relax
	\fi
	\CF@chemfig@v
}

\CF@def\CF@chemfig@v{%
	\let\CF@next@action\CF@chemfig@v% \`a prioi, on reboucle
	\ifx\CF@remain@molecule\@empty
		\let\CF@next@action\endgroup
	\else
		\CF@seek@submol
		\expandafter\CF@seek@node\expandafter{\CF@remain@molecule}\CF@current@atomgroup\CF@remain@molecule
		\ifx\@empty\CF@current@atomgroup% pas de noeud pour commencer ?
			\def\CF@bond@outnode{n\CF@last@groupnumber-%
				 \ifx\CF@current@fromatom\@empty
					 \ifdim\CF@current@angle pt<90pt \number\CF@cnt@atomingroup
					 \else\ifdim\CF@current@angle pt>270pt \number\CF@cnt@atomingroup\else1\fi
					 \fi
				 \else\CF@current@fromatom
				 \fi}%
			\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\CF@remain@molecule\relax\@nil
			\CF@if@firsttokin@i{-=<>~}% la suite est une liaison
				{\ifnum\CF@last@action=\tw@% c'est la deuxi\`eme liaison cons\'ecutive ?
					\CF@insert@emptygroup\CF@remain@molecule% ins\`ere un groupe vide
					\edef\CF@bond@outnode{\CF@bond@outnode}%
				\else
					\ifCF@incycle\advance\CF@cnt@cycle\@ne\fi
					\expandafter\CF@analyse@bond\expandafter{\CF@remain@molecule}\CF@bond@type
					\edef\CF@bond@outnode{\CF@bond@outnode}%
					\let\CF@remain@molecule\CF@remain@afterbond
					\ifCF@incycle
						\ifnum\CF@cnt@cycle=\CF@cycle@num\relax
							\expandafter\expandafter\expandafter\@firstoftwo
						\else
							\expandafter\expandafter\expandafter\@secondoftwo
						\fi
					\else
						\expandafter\@secondoftwo
					\fi
						{\let\CF@next@action\endgroup
						\CF@draw@bond\CF@bond@type{\CF@bond@outnode}{\CF@hook@cycle}\CF@previous@atomgroup\CF@hook@atomgroup
						}%
						{\node[at=(\CF@bond@outnode),shift=(\ifcase\CF@split@state\or180-\or-\fi\CF@current@angle:\CF@current@length*\CF@atom@sep)](CF@node){};
						\let\CF@previous@angle\CF@current@angle
						\let\CF@last@action\tw@
						}%
				\fi
				\ifx\CF@remain@molecule\@empty% plus rien apr\`es la liaison -> ins\`ere un groupe vide
					\CF@insert@emptygroup\CF@remain@molecule
				\fi
				}%
				{\edef\CF@bond@outnode{\CF@bond@outnode}% \'evalue le l'atome de d\'epart de liaison
				\ifx(\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi% une parenth\`ese pour commencer ?
					{\ifnum\CF@last@action=\tw@% il y avait une liaison juste avant ?
						\CF@insert@emptygroup\CF@remain@molecule
					\else
						\expandafter\CF@grab@submol\expandafter{\CF@remain@molecule}%
						\begingroup
							\ifCF@incycle\let\CF@last@action\thr@@\fi% on \'etait dans un cycle
							\CF@incyclefalse
							\aftergroup\CF@chemfig@v
							\def\CF@next@action{\expandafter\CF@chemfig@iv\expandafter{\CF@sub@mol}}%
					\fi
					}%
					{\ifx\CF@remain@molecule\@empty
						\let\CF@next@action\endgroup
					\else% ce qui reste apr\`es le noeud courant n'est pas vide, ne commence pas par "-=~", ni par une parenth\`ese
						\ifx*\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi% un cycle ?
						{\ifnum\CF@last@action=\tw@
							\CF@insert@emptygroup\CF@remain@molecule% ins\`ere un groupe vide
						\else
							\ifCF@incycle\let\CF@last@action\thr@@\fi% on \'etait dans un cycle
							\ifnum\CF@last@action=\thr@@\let\CF@lastcycle@num\CF@cycle@num\fi
							\CF@expafterarg@ntimes2\CF@if@firsttokmatch{\expandafter\@gobble\CF@remain@molecule}*% un 2\`e "*" ?
								{\CF@expafterarg@ntimes2{\def\CF@remain@molecule}{\expandafter\@gobble\CF@remain@molecule}% enl\`eve la 1er \'etoile
								\CF@expafterarg@ntimes2\CF@if@firsttokmatch{\expandafter\@gobble\CF@remain@molecule}[% un crochet ensuite ?
									{\expandafter\CF@cycle@parsepreamblewithoptarg\CF@remain@molecule\@nil% \begingroup inclus
									}%
									{\def\CF@cyclearc@startangle{0}\def\CF@cyclearc@endangle{360}%
									\let\CF@cyclearc@directtikz\@empty
									\expandafter\CF@cycle@parsepreamble\CF@remain@molecule\@nil% \begingroup inclus
									}%
								\CF@cyclearctrue
								}%
								{\expandafter\CF@cycle@parsepreamble\CF@remain@molecule\@nil% \begingroup inclus
								\CF@cyclearcfalse
								}%
							\CF@cnt@cycle\z@
							\edef\CF@hook@cycle{\CF@bond@outnode}%
							\let\CF@hook@atomgroup\CF@previous@atomgroup
							\CF@incycletrue
							\ifnum\CF@last@action=\thr@@
								\pgfmathparse{360/\CF@lastcycle@num-180}% c'est un cycle dans un cycle
							\else
								\pgfmathparse{-180/\CF@cycle@num-90+\CF@cycle@anglecorrection}%
							\fi
							\let\CF@initcycle@angle\pgfmathresult
							\ifCF@cyclearc% on doit tracer l'arc de cercle dans le cycle ?
								\pgfmathparse{\CF@cycle@inraduiscoeff*\CF@current@length*\CF@atom@sep/(2*tan(180/\CF@cycle@num))}%
								\let\CF@cyclearc@radius\pgfmathresult
								\pgfmathparse{\CF@current@angle+\CF@initcycle@angle+180/\CF@cycle@num+90}
								\let\CF@cyclearc@initangle\pgfmathresult
								\pgfmathparse{\CF@current@length*\CF@atom@sep/(2*sin(180/\CF@cycle@num))}%
								\node[at=(\CF@bond@outnode),shift=(\CF@cyclearc@initangle:\pgfmathresult pt)](arccenter){};% le centre de l'arc
								\node[at=(arccenter),shift=(\CF@cyclearc@startangle:\CF@cyclearc@radius pt)](initarc){};% le d\'ebut de l'arc
								\expandafter\draw\expandafter[\CF@cyclearc@directtikz](initarc) arc (\CF@cyclearc@startangle:\CF@cyclearc@endangle:\CF@cyclearc@radius pt);
							\fi
							\aftergroup\CF@chemfig@v
							\def\CF@next@action{\expandafter\CF@chemfig@iv\expandafter{\CF@sub@mol}}%
						\fi
						}%
						{\errmessage{Package \CF@package@name\space Error: something went wrong here: \detokenize\expandafter{\CF@remain@molecule}^^JIf you think it's a bug, please, send a Minimal Example to the author.}}%
					\fi}%
				}%
		\else
			\CF@expand@second{\CF@expand@second{\CF@expand@second\CF@draw@atomgroup\CF@current@angle}\CF@current@toatom}\CF@current@atomgroup
		\fi
	\fi
	\CF@next@action
}

\CF@def\CF@cycle@parsepreamble*#1#2\@nil{%
	\ifnum#1<\thr@@
		\errmessage{Package \CF@package@name\space Error: A cycle must be at least a triangle.^^JThe number following "*" must be 3 or more}%
	\fi
	\def\CF@remain@molecule{#2}%
	\expandafter\CF@grab@submol\expandafter{\CF@remain@molecule}%
	\begingroup
	\def\CF@cycle@num{#1}%
}

\CF@def\CF@cycle@parsepreamblewithoptarg*[#1]#2#3\@nil{%
	\CF@cycle@parseoptarg#1,\@empty,\@empty,\@empty\@nil
	\CF@cycle@parsepreamble*#2#3\@nil
}

\CF@def\CF@cycle@parseoptarg#1,#2,#3\@nil{%
	\ifx\@empty#1\@empty\def\CF@cyclearc@startangle{0}\else\def\CF@cyclearc@startangle{#1}\fi
	\ifx\@empty#2\@empty\def\CF@cyclearc@endangle{360}\else\def\CF@cyclearc@endangle{#2}\fi
	\expandafter\def\expandafter\CF@cyclearc@directtikz\expandafter{\CF@sanitize@lastitem#3,\@empty\@nil}%
}

\CF@def\CF@grab@submol#1{%
	\begingroup
		\catcode`(\@ne\catcode`)\tw@
		\expandafter\expandafter\expandafter
	\endgroup
	\expandafter\CF@grab@submol@i\scantokens{\relax#1}% le \relax sert \`a meubler pour ne pas que l'argument d\'elimit\'e n'enl\`eve les accolades
}

\CF@def\CF@grab@submol@i#1\@nil{%
	\expandafter\assign@tonil\expandafter\CF@remain@molecule\scantokens\expandafter\expandafter\expandafter{\expandafter\@gobble\@gobble#1}%
	\expandafter\assign@tonil\expandafter\CF@sub@mol\scantokens\expandafter\expandafter\expandafter{\expandafter\@car\@gobble#1\@nil}%
}

\CF@def\assign@tonil#1#2\@nil{\def#1{#2}}

\CF@def\CF@ifcar@isupperletter#1{%
	\ifcat\relax\noexpand#1%
		\let\CF@next\@secondoftwo% faux si c'est une sc
	\else
		\ifnum`#1<`A
			\let\CF@next\@secondoftwo
		\else
			\ifnum`#1>`Z
				\let\CF@next\@secondoftwo
			\else
				\let\CF@next\@firstoftwo
			\fi
		\fi
	\fi
	\CF@next
}

% Cr\'e\'e 4 noeuds au dessus et au dessous des noeuds #1 et #2
% \`a une distance de #3 du noeud #1 et #4 du noeud #2
\CF@def\CF@create@normnodes#1#2#3#4{%
	\ifx\@empty#3\@empty\else
		\node[at=(#1),xshift=#3*\CF@norm@x,yshift=#3*\CF@norm@y](#11){};
		\node[at=(#1),xshift=-#3*\CF@norm@x,yshift=-#3*\CF@norm@y](#12){};
	\fi
	\ifx\@empty#4\@empty\else
		\node[at=(#2),xshift=#4*\CF@norm@x,yshift=#4*\CF@norm@y](#21){};
		\node[at=(#2),xshift=-#4*\CF@norm@x,yshift=-#4*\CF@norm@y](#22){};
	\fi
}

\CF@def\CF@compute@nodevect#1#2{%
	\pgfextractx\CF@dim{\pgfpointanchor{#1}{center}}\edef\CF@dimax{\the\CF@dim}%
	\pgfextracty\CF@dim{\pgfpointanchor{#1}{center}}\edef\CF@dimay{\the\CF@dim}%
	\pgfextractx\CF@dim{\pgfpointanchor{#2}{center}}\edef\CF@dimbx{\the\CF@dim}%
	\pgfextracty\CF@dim{\pgfpointanchor{#2}{center}}\edef\CF@dimby{\the\CF@dim}%
	\pgfmathparse{veclen(\CF@dimbx-\CF@dimax,\CF@dimby-\CF@dimay)}\let\CF@len@vector\pgfmathresult
	\pgfmathparse{(\CF@dimay-\CF@dimby)/\CF@len@vector}\let\CF@norm@x\pgfmathresult
	\pgfmathparse{(\CF@dimbx-\CF@dimax)/\CF@len@vector}\let\CF@norm@y\pgfmathresult
}

\CF@def\CF@set@offset#1#2{%
	\ifx#1\@empty
		\edef#1{\ifx#2\CF@empty@node0pt\else\ifx#2\@empty0pt\else\CF@bond@offset\fi\fi}%
	\fi
}

\CF@def\CF@draw@bond#1#2#3#4#5{% #1=type de liaison #2 et #3:nom de noeuds de d\'ebut et fin #4 et #5: contenu des atomes de d\'ebut et fin
	\CF@set@offset\CF@start@offset#4%
	\CF@set@offset\CF@end@offset#5%
	\let\CF@current@bondstyle\CF@bond@style
	\unless\ifx\CF@current@tikz\@empty\CF@expadd@tocs\CF@current@bondstyle{\expandafter,\CF@current@tikz}\fi
	\path(#2)--(#3)coordinate[pos=0](#2@)coordinate[pos=1](#3@);%
	\CF@compute@nodevect{#2@}{#3@}%
	\pgfmathparse{\CF@start@offset/\CF@len@vector}\let\CF@start@coeff\pgfmathresult
	\pgfmathparse{1-\CF@end@offset/\CF@len@vector}\let\CF@end@coeff\pgfmathresult
	\path(#2@)--(#3@)coordinate[pos=\CF@start@coeff](#2@@)coordinate[pos=\CF@end@coeff](#3@@);%
	\unless\ifx\CF@movebond@name\@empty% on doit poser un nœud sur la liaison
		\path(#2@@)--(#3@@)coordinate[overlay,pos=\CF@movebond@coeff](\CF@movebond@name);
		\let\CF@movebond@name\@empty
	\fi
	\ifcase#1\relax
		\errmessage{Package \CF@package@name\space Error: unknown bond type, this error should not occur^^JIf you think it's a bug, send a Minimal Example to the author}%
	\or% 1 = liaison simple
		\CF@draw@bond@i(#2@@)--(#3@@);
	\or% 2 = liaison double
		\ifCF@incycle
			\ifnum\CF@doublebond@type=\z@
				\let\CF@doublebond@type\@ne
			\fi
			\ifnum\CF@split@state>\z@
				\let\CF@doublebond@type\tw@
			\fi
			\pgfmathparse{\CF@double@sep*tan(180/\CF@cycle@num)}%
			\let\CF@doublebond@lengthcorrection\pgfmathresult
		\fi
		\ifcase\CF@doublebond@type
			\CF@create@normnodes{#2@@}{#3@@}{\CF@double@sep/2}{\CF@double@sep/2}%
			\CF@draw@bond@i(#2@@1)--(#3@@1);
			\CF@draw@bond@i(#2@@2)--(#3@@2);
		\or
			\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
			\CF@draw@bond@i(#2@@)--(#3@@);
			\begingroup% ajuste \'eventuellement les longueurs des liaisons doubles
				\ifCF@incycle
					\ifdim\CF@start@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten <=\CF@doublebond@lengthcorrection pt}%
					\fi
					\ifdim\CF@end@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten >=\CF@doublebond@lengthcorrection pt}%
					\fi
				\fi
				\CF@draw@bond@i(#2@@1)--(#3@@1);
			\endgroup
		\or
			\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
			\CF@draw@bond@i(#2@@)--(#3@@);
			\begingroup% ajuste \'eventuellement les longueurs des liaisons doubles
				\ifCF@incycle
					\ifdim\CF@start@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten \ifnum\CF@split@state=\z@<=-\else>=\fi\CF@doublebond@lengthcorrection pt}%
					\fi
					\ifdim\CF@end@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten \ifnum\CF@split@state=\z@>=-\else<=\fi\CF@doublebond@lengthcorrection pt}%
					\fi
				\fi
				\CF@draw@bond@i(#2@@2)--(#3@@2);
			\endgroup
		\fi
	\or% 3 = liaison triple
		\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
		\CF@draw@bond@i(#2@@)--(#3@@);
		\CF@draw@bond@i(#2@@1)--(#3@@1);
		\CF@draw@bond@i(#2@@2)--(#3@@2);
	\or% 4 = liaison Cram pleine de #2 vers #3
		\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
		\expandafter\filldraw\expandafter[\CF@current@bondstyle,line join=bevel](#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
	\or% 5 = liaison Cram pleine de #3 vers #2
		\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
		\expandafter\filldraw\expandafter[\CF@current@bondstyle,line join=bevel](#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
	\or% 6 = liaison Cram pointill\'ee de #2 vers #3
		\scope
			\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
			\clip(#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
			\expandafter\draw\expandafter[\CF@current@bondstyle,dash pattern=on \CF@cram@dashlength off \CF@cram@dashsep,line width=\CF@cram@basewidth](#2@@)--(#3@@);
		\endscope
	\or% 7 = liaison Cram pointill\'ee de #3 vers #2
		\scope
			\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
			\clip(#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
			\expandafter\draw\expandafter[\CF@current@bondstyle,dash pattern=on \CF@cram@dashlength off \CF@cram@dashsep,line width=\CF@cram@basewidth](#3@@)--(#2@@);
		\endscope
	\or% 8 = liaison Cram triangle \'evid\'e de #2 vers #3
		\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
		\expandafter\draw\expandafter[\CF@current@bondstyle,line join=bevel](#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
	\or% 9 = liaison Cram triangle \'evid\'e de #3 vers #1
		\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
		\expandafter\draw\expandafter[\CF@current@bondstyle,line join=bevel](#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
	\else
		\errmessage{Package \CF@package@name\space Error: unknown bond type, this error should not occur^^JIf you think it's a bug, send a Minimal Example to the author}%
	\fi
	\let\CF@start@offset\@empty
	\let\CF@end@offset\@empty
}

\CF@def\CF@draw@bond@i{\expandafter\draw\expandafter[\CF@current@bondstyle]}

\CF@def\CF@hook@drawall{% dessine tous les crochets contenus dansla sc \CF@hook@draw
	\unless\ifx\CF@hook@drawlist\@empty
		\expandafter\CF@hook@drawfirst\CF@hook@drawlist\@nil% trace un lien de crochet \`a crochet
		\expandafter\CF@hook@drawall
	\fi
}

\CF@def\CF@hook@drawfirst[#1,#2,#3]#4#5#6#7#8\@nil{%
	\def\CF@hook@drawlist{#8}%
	\begingroup
		\def\CF@current@tikz{#3}%
		\def\CF@hook@startcontent{#6}\def\CF@hook@endcontent{#7}%
		\CF@if@integer{#2}%
			{\CF@draw@bond{#2}{#4}{#5}\CF@hook@startcontent\CF@hook@endcontent}%
			{\CF@bond@findnum{#2}\CF@bond@currentnum
			\CF@draw@bond\CF@bond@currentnum{#4}{#5}\CF@hook@startcontent\CF@hook@endcontent
			}%
	\endgroup
}

\CF@def\CF@extract@atom#1-#2\@nil{#2}% transforme le bound@outnode en n° de l'atome

\CF@def\setnodestyle{\def\CF@node@style}
\setnodestyle{}

\CF@def\setbondstyle{\def\CF@bond@style}
\setbondstyle{}

\expandafter\CF@def\expandafter\CF@gobble@movearg\string @#1#2\@nil#3%
{%
	\expandafter\def\csname atom@\number\CF@cnt@atomnumber\endcsname{#2}%
	\CF@if@instr{#1},%
		{\CF@analyse@movearg#1\@nil#3\let\CF@movebond@coeff\@empty}%
		{\def#3{#1}}%
	\ifx\@empty#2\@empty\let\CF@node@strut\@empty\fi
}%

\CF@def\hflipnext{\let\CF@split@state\@ne}

\CF@def\vflipnext{\let\CF@split@state\tw@}
\let\CF@split@state\z@

\CF@def\CF@draw@atomgroup#1#2#3{% #1=angle d'arriv\'ee de la liaison #2=numero atome sur lequel arrive la liaison #3=groupe d'atomes
	\expandafter\let\expandafter\CF@bond@outcontent% assigne le contenu de l'atome d'o\`u part la liaison
		\csname
			\ifdefined\CF@bond@outnode
				atom@\expandafter\CF@extract@atom\CF@bond@outnode\@nil
			\else
				@empty%
			\fi
		\endcsname
	\global\advance\CF@cnt@groupnumber\@ne
	\let\CF@current@atom\@empty
	\global\let\CF@hook@drawlist\@empty
	\CF@cnt@atomingroup\z@
	\CF@if@firsttokmatch{#3}?{\CF@draw@atomgroup@i{{}#3}}{\CF@draw@atomgroup@i{#3}}%
	\def\CF@current@atomgroup{#3}%
	\CF@remove@movearg\CF@current@atomgroup% enl\`eve les "@{<nom>}"
	\CF@if@instr{#3}?%
		{\CF@remove@hook\CF@current@atomgroup
		\ifx\@empty\CF@current@atomgroup\let\CF@current@atomgroup\CF@empty@node\fi}%
		\relax
	\ifx\@empty#2\@empty%
	\else
		\ifnum#2<\@ne
			\immediate\write\CF@unused{Package \CF@package@name\space Warning: no atom found at position #2, pershaps you mispelled the optional argument of the bond.}%
		\else
			\ifnum#2>\CF@cnt@atomingroup
				\errmessage{Package \CF@package@name\space Error: no atom found at position #2, pershaps you mispelled the optional argument of the bond.}%
			\fi
		\fi
	\fi
	\edef\CF@hook@atomnumber{%
		\ifx\@empty#2\@empty
			\ifdim#1pt>90pt
				\ifdim#1pt<270pt \number\CF@cnt@atomingroup\else1\fi
			\else1%
			\fi
		\else#2%
		\fi}%
	\CF@cnt@atomnumber\CF@hook@atomnumber
	\ifx\CF@current@atomgroup\CF@empty@node
		\let\CF@node@strut\@empty
	\else
		\ifx\@empty\CF@bond@outcontentsaved
			\def\CF@node@strut{\vphantom\CF@bond@outcontent}%
		\else
			\def\CF@node@strut{\vphantom\CF@bond@outcontentsaved}%
		\fi
	\fi
	\edef\CF@opt@string{anchor=\ifnum\CF@last@action=\z@ base\else center\fi,at=(CF@node),\CF@node@style}% premier atome de la mol\'ecule affich\'e
	\loop
		\unless\ifnum\CF@cnt@atomnumber>\CF@cnt@atomingroup
		\expandafter\expandafter\expandafter\futurelet\expandafter\expandafter\expandafter\CF@toks@a\expandafter\expandafter\expandafter
			\CF@gobble@tonil\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil
		\expandafter\ifx\string @\CF@toks@a% l'atome courant commence par un "@"
			\expandafter\expandafter\expandafter\CF@gobble@movearg\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil\CF@moveatom@name
			\expandafter\node\expandafter[\CF@opt@string,overlay](\CF@moveatom@name){\phantom{\CF@node@content}};%
			\let\CF@moveatom@name\@empty
		\fi
		\expandafter\node\expandafter[\CF@opt@string](n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber){\CF@node@content};%
		\let\CF@node@strut\@empty
		\advance\CF@cnt@atomnumber\@ne
		\edef\CF@opt@string{anchor=base \ifnum\CF@split@state=\@ne east\else west\fi,at=(n\number\CF@cnt@groupnumber-\number\numexpr\CF@cnt@atomnumber-1.base \ifnum\CF@split@state=\@ne west\else east\fi),\CF@node@style}%
	\repeat
	\CF@cnt@atomnumber\CF@hook@atomnumber
	\ifnum\CF@last@action=\tw@% s'il faut tracer une liaison
		\gdef\CF@cycle@anglecorrection{0}% alors c'est qu'un cycle ne peut pas commencer la mol\'ecule : annulation de la correction d'angle
		\CF@draw@bond\CF@bond@type{\CF@bond@outnode}{n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber}\CF@previous@atomgroup\CF@current@atomgroup
	\fi
	\let\CF@last@action\@ne% met la derni\`ere action \`a 1 : affichage d'un noeud
	\loop
		\ifnum\CF@cnt@atomnumber>\@ne
		\advance\CF@cnt@atomnumber\m@ne
		\edef\CF@opt@string{anchor=base \ifnum\CF@split@state=\@ne west\else east\fi,at=(n\number\CF@cnt@groupnumber-\number\numexpr\CF@cnt@atomnumber+1.base \ifnum\CF@split@state=\@ne east\else west\fi),\CF@node@style}%
		\expandafter\expandafter\expandafter\futurelet\expandafter\expandafter\expandafter\CF@toks@a\expandafter\expandafter\expandafter
			\CF@gobble@tonil\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil
		\expandafter\ifx\string @\CF@toks@a% l'atome courant commence par un "@"
			\expandafter\expandafter\expandafter\CF@gobble@movearg\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil\CF@moveatom@name
			\expandafter\node\expandafter[\CF@opt@string,overlay](\CF@moveatom@name){\phantom{\CF@node@content}};%
			\let\CF@moveatom@name\@empty
		\fi
		\expandafter\node\expandafter[\CF@opt@string](n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber){\CF@node@content};%
	\repeat
	\CF@hook@drawall
	\edef\CF@last@groupnumber{\number\CF@cnt@groupnumber}%
	\let\CF@previous@atomgroup\CF@current@atomgroup
}

\expandafter\CF@def\expandafter\CF@keep@movearg\string @#1#2\@nil{\expandafter\def\expandafter\CF@current@atom\expandafter{\string @{#1}}}

\CF@def\CF@draw@atomgroup@i#1{% transforme #1 en un groupe d'atomes
	\ifx\@empty#1\@empty
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
	\else
		\advance\CF@cnt@atomingroup\@ne
		\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
		\expandafter\ifx\string @\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\CF@keep@movearg#1\@nil
			\CF@swap@fi
			\CF@remove@movearg@i#1\@nil\CF@after@movearg
			\expandafter\CF@draw@atomgroup@ii\expandafter{\CF@after@movearg}%
			}%
			{\CF@swap@fi
			\let\CF@current@atom\@empty
			\CF@draw@atomgroup@ii{#1}%
			}%
	\fi
}

\CF@def\CF@draw@atomgroup@ii#1{%
	\ifx\@empty#1\@empty
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
	\else
	\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
	\ifx\bgroup\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\CF@expadd@tocs\CF@current@atom{\expandafter{\@car#1\@nil}}%
		\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
		}%
		{\ifx\@sptoken\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\CF@add@tocs\CF@current@atom{ }%
			\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@space#1\@nil}%
			}%
			{\CF@expadd@tocs\CF@current@atom{\@car#1\@nil}%
			\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
			}%
		}%
	\fi
}

% enl\`eve tous les "@{nom}" de la sc #1
\CF@def\CF@remove@movearg#1{%
	\CF@expand@afterfirst{\expandafter\CF@if@instr\expandafter{#1}}{\string @}%
		{\expandafter\CF@remove@movearg@i#1\@nil#1%
		\CF@remove@movearg#1}%
		\relax
}

% enl\`eve le premier "@{<nom>}" de l'argument et l'assigne \`a #2
\CF@def\CF@remove@movearg@i#1\@nil#2{%
	\expandafter\def\expandafter\CF@remove@movearg@ii\expandafter##\expandafter1\string @{%
		\expandafter\def\expandafter#2\expandafter{\@gobble##1}% mange le \relax
		\CF@remove@movearg@iii\relax
	}%
	\def\CF@remove@movearg@iii##1\@nil{\CF@expadd@tocs#2{\@gobbletwo##1}}% mange le \relax et le <nom>
	\CF@remove@movearg@ii\relax#1\@nil
}

\CF@def\CF@draw@atomgroup@iii#1{% transforme #1 en un groupe d'atomes
	\ifx\@empty#1\@empty%
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
		\let\CF@current@atom\@empty
	\else
		\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
		\expandafter\ifx\string @\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
			\let\CF@current@atom\@empty
			\CF@swap@fi\CF@draw@atomgroup@i{#1}%
			}%
			{\ifx|\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
				{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
				\let\CF@current@atom\@empty
				\CF@swap@fi\expandafter\CF@draw@atomgroup@i\expandafter{\@gobble#1}%
				}%
				{\ifx\@sptoken\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
					{\CF@add@tocs\CF@current@atom{ }%
					\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@space#1\@nil}%
					 }%
					{\ifx\bgroup\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
						{\CF@expadd@tocs\CF@current@atom{\expandafter{\@car#1\@nil}}%
						\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
						}%
						{\expandafter\CF@ifcar@isupperletter\expandafter{\@car#1\@nil}%
							{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
							\let\CF@current@atom\@empty
							\CF@swap@fi\CF@draw@atomgroup@i{#1}%
							}%
							{\ifx?\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
								{\expandafter\CF@if@firsttokmatch\expandafter{\@gobble#1}[% un crochet apr\`es le "?"
									{\expandafter\CF@grab@optarg\@gobble#1\@nil\CF@after@hook}%
									{\expandafter\CF@grab@optarg\expandafter[\expandafter]\@gobble#1\@nil\CF@after@hook}%
									\CF@expand@second{\CF@expand@second\CF@if@instr\CF@hook@list}{\expandafter(\CF@hook@currentname)}% crochet d\'ej\`a d\'efini ?
									{\expandafter\CF@hook@parselist\expandafter{\CF@hook@currentname}% va chercher les caract\'eristiques du crochet sauvegard\'e
									\CF@edefadd@tocs\CF@hook@drawlist{%
										[\CF@hook@currentname,\CF@hook@currentlink,\CF@hook@currenttikz]{\CF@hook@savedcoord}{n\number\CF@cnt@groupnumber-\number\CF@cnt@atomingroup}}%
									\CF@expadd@tocs\CF@hook@drawlist{\expandafter{\CF@hook@savedcontent}}%
									\CF@expadd@tocs\CF@hook@drawlist{\expandafter{\CF@current@atom}}% ajoute les 4 arguments \`a la liste des crochets \`a tracer
									\global\let\CF@hook@drawlist\CF@hook@drawlist
									}%
									{\CF@edefadd@tocs\CF@hook@list{(\CF@hook@currentname)|n\number\CF@cnt@groupnumber-\number\CF@cnt@atomingroup|}%
									\CF@expadd@tocs\CF@hook@list{\CF@current@atom|}%
									\global\let\CF@hook@list\CF@hook@list
									}%
								\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@hook}%
								}%
								{\CF@expadd@tocs\CF@current@atom{\@car#1\@nil}%
								\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
								}%
							}%
						}%
					}%
				}%
			}%
	\fi
}

\CF@def\CF@kook@defaultname{a}
\CF@def\CF@hook@defaultlink{-}
\CF@def\CF@hook@defaulttikz{}

\CF@def\CF@hook@parseoptarg#1,#2,#3\@nil{%
	\CF@testempty@andassign\CF@hook@currentname{#1}\CF@kook@defaultname
	\CF@testempty@andassign\CF@hook@currentlink{#2}\CF@hook@defaultlink
	\CF@testempty@andassign\CF@hook@currenttikz{#3}\CF@hook@defaulttikz
}

\CF@def\CF@grab@optarg[#1]#2\@nil#3{%
	\CF@hook@parseoptarg#1,,\@nil
	\def#3{#2}%
}

\CF@def\CF@hook@parselist#1{% #1 est le nom du noeud \`a retrouver
	\def\CF@hook@parselist@i##1(#1)|##2|##3|##4\@nil{%
		\def\CF@hook@savedcoord{##2}\def\CF@hook@savedcontent{##3}%
	}%
	\expandafter\CF@hook@parselist@i\CF@hook@list\@nil
}

\CF@def\CF@remove@hook#1{% enl\`eve tous les crochets (et leurs arguments optionnels) de la sc #1
	\expandafter\CF@if@instr\expandafter{#1}{?[}%
		{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#1%
			\expandafter\expandafter\expandafter{\expandafter\CF@remove@opthook#1\@nil}%
		\CF@remove@hook#1%
		}%
		{\CF@remove@hook@i#1}%
}

\CF@def\CF@remove@hook@i#1{%
	\expandafter\CF@if@instr\expandafter{#1}?%
		{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#1%
			\expandafter\expandafter\expandafter{\expandafter\CF@remove@singlehook#1\@nil}%
		\CF@remove@hook@i#1%
		}%
		\relax
}

\CF@def\CF@remove@opthook#1?[#2]#3\@nil{#1#3}

\CF@def\CF@remove@singlehook#1?#2\@nil{#1#2}

\CF@def\setlewis{\@testopt\CF@setlewis{0.3ex}}

\CF@def\CF@setlewis[#1]#2#3#4{%
	\def\CF@lewis@widthdouble{#1}%
	\ifx\@empty#2\@empty\def\CF@lewis@offset{0.4ex}\else\def\CF@lewis@offset{#2}\fi
	\ifx\@empty#3\@empty\def\CF@lewis@length{1.5ex}\else\def\CF@lewis@length{#3}\fi
	\ifx\@empty#4\@empty\def\CF@lewis@style{}\else\def\CF@lewis@style{#4}\fi
}
\setlewis{}{}{}

\CF@def\setlewisdist#1{%
	\def\CF@lewis@dist{#1}\ifx\@empty\CF@lewis@dist\def\CF@lewis@dist{0.2em}\fi
}
\setlewisdist{0.3em}

\CF@def\Lewis{\@testopt{\CF@lewis@i{}}{1}}

\CF@def\lewis{\@testopt{\CF@lewis@i{,overlay}}{1}}

\CF@def\CF@lewis@i#1[#2]{%
	\def\CF@lewis@diagcoeff{#2}%
	\ifx\@empty\CF@lewis@diagcoeff\def\CF@lewis@diagcoeff{1}\fi
	\CF@lewis@ii{#1}}

\CF@def\CF@lewis@ii#1#2{\CF@lewis@iii#2\@nil{#1}}

\CF@def\CF@lewis@iii#1,#2\@nil#3{%
	\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
		\@makeother;\@makeother:%
		\setbox\CF@lewis@box\hbox{\printatom{#2}}%
		\node(CF@lewis@anchor){};
		\def\CF@lewis@remainpos{#1}%
		\let\CF@lewis@previouspos\@empty
		\loop
			\unless\ifx\CF@lewis@remainpos\@empty
				\edef\CF@lewis@currentpos{\expandafter\@car\CF@lewis@remainpos\@nil}%
				\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
				\pgfmathparse{\wd\CF@lewis@box/2+\ifcase\CF@lewis@currentpos\space1\or1\or0\or-1\or-1\or-1\or0\or1\fi*(\wd\CF@lewis@box/2)}%
				\let\CF@lewis@x\pgfmathresult
				\pgfmathparse{\ht\CF@lewis@box/2+\ifcase\CF@lewis@currentpos\space0\or1\or1\or1\or0\or-1\or-1\or-1\fi*(\ht\CF@lewis@box/2\ifnum\CF@lewis@currentpos>4 +\dp\CF@lewis@box\fi)}%
				\let\CF@lewis@y\pgfmathresult
				\edef\CF@lewis@xoffset{\ifcase\CF@lewis@currentpos\space1\or0.70711\or0\or-0.70711\or-1\or-0.70711\or0\or0.70711\fi}%
				\edef\CF@lewis@yoffset{\ifcase\CF@lewis@currentpos\space0\or0.70711\or1\or0.70711\or0\or-0.70711\or-1\or-0.70711\fi}%
				\ifodd\CF@lewis@currentpos\relax
					\pgfmathparse{\CF@lewis@offset*\CF@lewis@diagcoeff}\let\CF@lewis@current@offset\pgfmathresult
				\else
					\let\CF@lewis@current@offset\CF@lewis@offset
				\fi
				\if.\expandafter\@car\CF@lewis@remainpos\relax\@nil
					\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
					\CF@expand@afterfirst{\draw[fill,black,}{\CF@lewis@style#3]}%
						(\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset,\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset)circle(0.15ex);%
				\else
					\if|\expandafter\@car\CF@lewis@remainpos\relax\@nil
						\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
						\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
						\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
						\expandafter\draw\expandafter[\CF@lewis@style#3]%
							(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt)--
							(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt+\CF@lewis@xoffset*\CF@lewis@widthdouble,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt+\CF@lewis@yoffset*\CF@lewis@widthdouble)--
							(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt+\CF@lewis@xoffset*\CF@lewis@widthdouble,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt+\CF@lewis@yoffset*\CF@lewis@widthdouble)--
							(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt)--cycle;%
					\else
						\if:\expandafter\@car\CF@lewis@remainpos\relax\@nil
							\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
							\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
							\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
							\CF@expand@afterfirst{\draw[fill,black,}{\CF@lewis@style#3]}%
								(\CF@lewis@x pt+\CF@lewis@dist*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@dist*\CF@lewis@xoffset/2 pt)circle(0.15ex)%
								(\CF@lewis@x pt-\CF@lewis@dist*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@dist*\CF@lewis@xoffset/2 pt)circle(0.15ex);%
						\else
							\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
							\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
							\expandafter\draw\expandafter[\CF@lewis@style#3]%
								(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt)--%
								(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt);%
						\fi
					\fi
			\fi
		\repeat
		\node[anchor=base west]at(CF@lewis@anchor){\box\CF@lewis@box};%
	\endtikzpicture
}

\CF@def\Chembelow{\begingroup\let\CF@tmp@str\@gobble\CF@chembelow@i}

\CF@def\chembelow{\begingroup\let\CF@tmp@str\@firstofone\CF@chembelow@i}

\CF@def\CF@chembelow@i{\@testopt\CF@chembelow@ii{1.5pt}}

\CF@def\CF@chembelow@ii[#1]#2#3{%
	\setbox\CF@box@boxa\hbox{\printatom{#2}}\setbox\CF@box@boxb\hbox{\printatom{#3}}%
	\vtop{%
		\hbox{\printatom{#2}}%
		\hrule width\z@ depth\z@ height#1
		\hbox to\wd\CF@box@boxa{\hss\printatom{#3}\hss}%
		\CF@tmp@str{\hrule width\z@ depth\z@ height-\dimexpr\ht\CF@box@boxb+\dp\CF@box@boxb+#1\relax}%
		}%
	\endgroup
}

\CF@def\Chemabove{\begingroup\let\CF@tmp@str\@gobble\CF@chemabove@i}

\CF@def\chemabove{\begingroup\let\CF@tmp@str\@firstofone\CF@chemabove@i}

\CF@def\CF@chemabove@i{\@testopt\CF@chemabove@ii{1.5pt}}

\CF@def\CF@chemabove@ii[#1]#2#3{%
	\setbox\CF@box@boxa\hbox{\printatom{#2}}\setbox\CF@box@boxb\hbox{\printatom{#3}}%
	\vbox{%
		\CF@tmp@str{\hrule width\z@ depth\z@ height-\dimexpr\ht\CF@box@boxb+\dp\CF@box@boxb+#1\relax}%
		\hbox to\wd\CF@box@boxa{\hss\printatom{#3}\hss}%
		\hrule width\z@ depth\z@ height#1
		\hbox{\printatom{#2}}%
	}%
	\endgroup
}

%%%%%% les signes et les fl\`eches
\CF@def\chemsign{\@testopt\CF@chemsign{0.5em}}

\CF@def\CF@chemsign[#1]#2{\hbox{\kern#1\relax#2\kern#1}}

\CF@def\setchemrel#1#2#3{%
	\ifx\@empty#1\@empty\def\CF@chemrel@vsep{2pt}\else\def\CF@chemrel@vsep{#1}\fi
	\ifx\@empty#2\@empty\def\CF@chemrel@hsep{0.7em}\else\def\CF@chemrel@hsep{#2}\fi
	\ifx\@empty#3\@empty\def\CF@chemrel@length{4em}\else\def\CF@chemrel@length{#3}\fi
}

\setchemrel{}{}{}

\CF@def\chemrel{\@testopt\CF@chemchemrel@i{}}

\CF@def\CF@chemchemrel@i[#1]{\@testopt{\CF@chemchemrel@ii[#1]}{}}

\CF@def\CF@chemchemrel@ii[#1][#2]#3{%
	\def\CF@chemrel@stuff
		{\leavevmode\kern\CF@chemrel@hsep
		\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
			\CF@if@instr{#3}{<>}%
				{\node[yshift=-1pt] at(0,0)(chemrel@start){\vphantom I};\node[yshift=-1pt] at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\expandafter\draw\expandafter[\CF@remove@equichars#3,\@nil-](chemrel@end)--(chemrel@start);\fill (chemrel@start)--++(4pt,-1.75pt)--+(-1.5pt,1.75pt)--cycle;%
				\node[yshift=1pt] at(0,0)(chemrel@start){\vphantom I};\node[yshift=1pt] at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\expandafter\draw\expandafter[\CF@remove@equichars#3,\@nil-](chemrel@start)--(chemrel@end);\fill(chemrel@end)--++(-4pt,1.75pt)--+(1.5pt,-1.75pt)--cycle;
				}%
				{\node at(0,0)(chemrel@start){\vphantom I};\node at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\draw[#3](chemrel@start)--(chemrel@end);%
				}%
		\endtikzpicture
		\kern\CF@chemrel@hsep
		}%
	\ifx\@empty#1\@empty
		\ifx\@empty#2\@empty\CF@chemrel@stuff
		\else\chembelow[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#2}}%
		\fi
	\else
		\ifx\@empty#2\@empty\chemabove[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#1}}%
		\else\chemabove[\CF@chemrel@vsep]{\chembelow[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#2}}}{\hbox{#1}}%
		\fi
	\fi
}

\CF@def\CF@remove@equichars#1<>#2\@nil{#1#2}

\CF@def\chemmove{%
	\@testopt\CF@chemmove{}}

\CF@def\CF@chemmove[#1]#2{%
	\ifx\@empty#2\@empty
		\expandafter\@gobble
	\else
		\expandafter\@firstofone
	\fi
	{\expandafter\tikzpicture\romannumeral\ifx\@empty#1\@empty\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\z@[remember picture,overlay]}{\z@[remember picture,overlay,#1]}#2
		\endtikzpicture
	}%
}

\CF@def\chemnameinit#1{%
	\setbox\CF@stuff@box\hbox{#1}%
	\edef\CF@dp@max{\the\dp\CF@stuff@box}%
}
\chemnameinit{}

\CF@def\CF@parse@molname#1\\#2\@nil{%
	\hbox to\CF@wd@stuffbox{\hss#1\hss}%
	\ifx\@empty#2\@empty
	\else
		\CF@swap@fi
		\CF@parse@molname#2\@nil
	\fi
}

\CF@def\chemname{%
	\@testopt\CF@chemname{1.5ex}%
}

\CF@def\CF@chemname[#1]#2#3{%
	\setbox\CF@stuff@box\hbox{#2}%
	\edef\CF@wd@stuffbox{\the\wd\CF@stuff@box}\edef\CF@dp@stuffbox{\the\dp\CF@stuff@box}%
	\leavevmode
	\ifdim\CF@dp@max<\CF@dp@stuffbox\let\CF@dp@max\CF@dp@stuffbox\fi
	\vtop{%
		\box\CF@stuff@box
		\nointerlineskip
		\kern\dimexpr#1+\CF@dp@max-\CF@dp@stuffbox\relax
		\CF@parse@molname#3\\\@nil
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    S C H E M A S      R E A C T I O N N E L S    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcount\CF@compound@cnt

\newdimen\CF@arrow@size

\newif\ifCF@name@start
\newif\ifCF@name@end
\newif\ifCF@reac@debug

\let\CF@scheme@nest\z@% ne PAS modifier cette ligne !

\CF@def\CF@subscheme{\@testopt\CF@subscheme@i{}}
\CF@def\CF@subscheme@i[#1]{\@testopt{\CF@subscheme@ii[#1]}{text}}
\CF@def\CF@subscheme@ii[#1][#2]#3{\schemestart[#1][#2]#3\schemestop}

\CF@def\schemedebug#1{% #1=true ou false
	\ifcsname CF@reac@debug#1\endcsname\csname CF@reac@debug#1\endcsname\else\CF@reac@debugfalse\fi
}
\schemedebug{false}

\CF@def\setcompoundstyle{\def\CF@default@compound@style}
\setcompoundstyle{}

\CF@def\CF@set@arrow@style#1,#2,#3\@nil#4#5#6{%
	\def#4{#1}%
	\expandafter\def\expandafter#5\expandafter{#2}%
	\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#6\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#3,\@empty\@nil}%
}

\CF@def\setarrowdefault#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@default@arrow@angle\CF@default@arrow@length\CF@default@arrow@style
	\ifx\@empty\CF@default@arrow@angle\def\CF@default@arrow@angle{0}\fi
	\ifx\@empty\CF@default@arrow@length\def\CF@default@arrow@length{1}\fi
}
\setarrowdefault{}

\CF@def\setarrowoffset#1{\def\CF@arrow@offset{#1}\ifx\CF@arrow@offset\@empty\def\CF@arrow@offset{1em}\fi}
\setarrowoffset{}

\CF@def\setcompoundsep#1{\def\CF@compound@sep{#1}\ifx\CF@compound@sep\@empty\def\CF@compound@sep{5em}\fi}
\setcompoundsep{}

\CF@def\setarrowlabelsep#1{\def\CF@arrow@labelsep{#1}\ifx\CF@arrow@labelsep\@empty\def\CF@arrow@labelsep{3pt}\fi}
\setarrowlabelsep{}

\CF@def\chemleft#1#2\chemright#3{%
	\leavevmode
	\begingroup
		\setbox\z@\hbox{$\vcenter{\hbox{}}$}\edef\CF@delim@math@ht{\the\ht\z@}%
		\setbox\z@\hbox{#2}\edef\CF@delim@dim{\the\dimexpr(\ht\z@+\dp\z@)/\tw@}%
		\edef\CF@delim@shift{\the\dimexpr(\ht\z@-\dp\z@)/\tw@-\CF@delim@math@ht}%
		\raise\CF@delim@shift\hbox{$\left#1\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right.$}\unhbox\z@
		\raise\CF@delim@shift\hbox{$\left.\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right#3$}%
	\endgroup
}

\CF@def\chemright#1{%
	\immediate\write\CF@unused{Package \CF@package@name\space Warning: "\string\chemright\string#1"ignored! No \string\chemleft\space previously found.^^J}%
}

\CF@def\chemup#1#2\chemdown#3{%
	\begingroup
		\setbox\z@\hbox{\printatom{#2}}\edef\CF@delim@dim{\the\dimexpr\wd\z@/\tw@}%
		\tikzpicture[every node/.style={inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
			\node[anchor=base west](chem@stuff){\unhbox\z@};%
			\node[at=(chem@stuff.north),anchor=east,rotate=-90]{$\left#1\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right.$};%
			\node[at=(chem@stuff.south),anchor=west,rotate=-90]{$\left.\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right#3$};%
		\endtikzpicture
	\endgroup
}

\CF@def\chemdown#1{%
	\immediate\write\CF@unused{Package \CF@package@name\space Warning: "\string\chemdown\string#1" ignored! No \string\chemup\space previously found.^^J}%
}

\CF@def\CF@and{\futurelet\CF@toks@a\CF@and@i}

\CF@def\CF@and@i{%
	\ifx\CF@toks@a\bgroup
		\expandafter\CF@and@ii
	\else
		\expandafter\CF@and@ii\expandafter{\expandafter}%
	\fi
}

\CF@def\CF@and@ii#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@signspace@ante\CF@signspace@post\CF@sign@vshift
	\ifx\@empty\CF@signspace@ante\let\CF@signspace@ante\CF@signspace@ante@default\fi
	\ifx\@empty\CF@signspace@post\let\CF@signspace@post\CF@signspace@post@default\fi
	\ifx\@empty\CF@sign@vshift\let\CF@sign@vshift\CF@sign@vshift@default\fi
	\raise\CF@sign@vshift\hbox{\kern\CF@signspace@ante$+$\kern\CF@signspace@post}%
}

\CF@def\setandsign#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@signspace@ante@default\CF@signspace@post@default\CF@sign@vshift@default
	\ifx\@empty\CF@signspace@ante@default\def\CF@signspace@ante@default{.5em}\fi
	\ifx\@empty\CF@signspace@post@default\def\CF@signspace@post@default{.5em}\fi
	\ifx\@empty\CF@sign@vshift@default\let\CF@sign@vshift@default\z@\fi
}
\setandsign{}

\CF@def\schemestart{%
	\xdef\CF@scheme@nest{\number\numexpr\CF@scheme@nest+\@ne}%
	\@testopt\CF@schemestart@i{}%
}

\CF@def\CF@schemestart@i[#1]{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@arrow@angle\CF@arrow@length\CF@arrow@style
	\ifx\@empty\CF@arrow@angle\let\CF@arrow@angle\CF@default@arrow@angle\fi
	\ifx\@empty\CF@arrow@length\let\CF@arrow@length\CF@default@arrow@length\fi
	\ifx\@empty\CF@arrow@style
		\let\CF@arrow@style\CF@default@arrow@style
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@arrow@style\expandafter\expandafter\expandafter
			{\expandafter\CF@default@arrow@style\expandafter,\CF@arrow@style}% se rajoute apr\`es le style par d\'efaut
	\fi
	\ifCF@reac@debug
		\tikzpicture[every node/.style={draw,anchor=base,inner sep=\z@,outer sep=\z@,minimum size=1.5pt},baseline,remember picture]%
	\else
		\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline,remember picture]%
	\fi
	\let\+\CF@and
	\let\arrow\CF@arrow
	\let\schemestop\CF@schemestop
	\let\subscheme\CF@subscheme
	\@testopt{\CF@schemestart@ii[#1]}{text}%
}

\CF@def\CF@schemestart@ii[#1][#2]{%
	\ifnum\CF@scheme@nest=\@ne% la commande n'est pas imbriqu\'ee ?
		\CF@compound@cnt\z@
	\fi
	\edef\CF@current@nodename{c\number\CF@compound@cnt}%
	\let\CF@next@nodename\@empty
	\let\CF@next@nodestyle\@empty
	\let\CF@direct@arrow@list\@empty
	\ifCF@reac@debug
		\node[fill,green](\CF@current@nodename){};%
	\else
		\node(\CF@current@nodename){};%
	\fi
	\def\CF@next@nodeanchor{#2}%
	\ifx\CF@next@nodeanchor\@empty\def\CF@next@nodeanchor{text}\fi
	\let\CF@compound\@empty
	\CF@schemestart@iii
}

\CF@def\CF@schemestart@iii{%
	\futurelet\CF@toks@a\CF@schemestart@v% va sentir le prochain token...
}

{\def\:{\CF@schemestart@iv}\expandafter}\expandafter\CF@def\: {\futurelet\CF@toks@a\CF@schemestart@v}

\CF@def\CF@schemestart@v{% ... et l'examine :
	\CF@if@firsttokin@i{\arrow\schemestop\merge}%
		\relax
		{\ifx\CF@toks@a\bgroup
			\let\CF@next@action\CF@add@nextarg
		\else
			\ifx\CF@toks@a\@sptoken
				\CF@add@tocs\CF@compound{ }%
				\let\CF@next@action\CF@schemestart@iv
			\else
				\def\CF@next@action{\CF@add@tocs\CF@compound}%
				\afterassignment\CF@schemestart@iii
			\fi
		\fi
		\CF@next@action}%
}

\CF@def\CF@add@nextarg#1{\CF@add@tocs\CF@compound{{#1}}\CF@schemestart@iii}

\CF@def\CF@display@compound#1#2{% #1 = nom et #2 = style
	\unless\ifx\@empty\CF@compound
		\global\advance\CF@compound@cnt\@ne
		\ifx\CF@default@compound@style\@empty
			\let\CF@current@nodestyle\@empty
		\else
			\expandafter\def\expandafter\CF@current@nodestyle\expandafter{\CF@default@compound@style,}%
		\fi
		\CF@add@tocs\CF@current@nodestyle{anchor=\CF@next@nodeanchor,at=(\CF@current@nodename)}%
		\ifx\@empty#2\@empty
			\unless\ifx\CF@next@nodestyle\@empty
				\CF@expadd@tocs\CF@current@nodestyle{\expandafter,\CF@next@nodestyle}%
			\fi
		\else
			\unless\ifx\CF@next@nodestyle\@empty
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: two styles for the same node, first style "\CF@next@nodestyle" ignored^^J}%
			\fi
			\CF@add@tocs\CF@current@nodestyle{,#2}%
		\fi
		\ifx\@empty#1\@empty
			\edef\CF@tmp@str{\ifx\CF@next@nodename\@empty c\number\CF@compound@cnt\else\CF@next@nodename\fi}%
		\else
			\unless\ifx\CF@next@nodename\@empty
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: two names for the same node, first name "\CF@next@nodename" ignored^^J}%
			\fi
			\edef\CF@tmp@str{#1}%
		\fi
		\expandafter\node\expandafter[\CF@current@nodestyle](\CF@tmp@str){\CF@compound};%
		\ifCF@reac@debug
			\node[draw=none,anchor=270,at=(\CF@tmp@str.90),fill=green!60,overlay,opacity=0.5]{\scriptsize\bfseries\CF@tmp@str};%
		\fi
		\let\CF@current@nodename\CF@tmp@str
	\fi
}

\CF@def\CF@schemestop{%
	\CF@display@compound{}{}%
	\CF@direct@arrow@list
	\endtikzpicture
	\xdef\CF@scheme@nest{\number\numexpr\CF@scheme@nest-\@ne}%
}

\CF@def\CF@analyse@arrowarg#1{\CF@analyse@arrowarg@i#1[]\@nil}

\CF@def\CF@analyse@arrowarg@i#1[#2]#3\@nil{%
	\CF@if@instr{#1}.{\CF@add@tocs\CF@tmp@str{#1[#2]}}{\CF@add@tocs\CF@tmp@str{#1.[#2]}}%
}

\CF@def\CF@arrow{%
	\@ifnextchar(%
		\CF@arrow@i
		{\@ifnextchar\bgroup{\CF@arrow@ii(.[]--.[])}{\CF@arrow@ii(.[]--.[]){}}}%
}

\CF@def\CF@arrow@i(#1--#2){%
	\def\CF@tmp@str{(}%
	\CF@analyse@arrowarg{#1}%
	\CF@add@tocs\CF@tmp@str{--}%
	\CF@analyse@arrowarg{#2}%
	\CF@add@tocs\CF@tmp@str)%
	\@ifnextchar\bgroup{\expandafter\CF@arrow@ii\CF@tmp@str}{\expandafter\CF@arrow@ii\CF@tmp@str{}}%
}

\CF@def\CF@arrow@ii(#1.#2[#3]--#4.#5[#6])#7{%
	\def\CF@current@arrowtype{#7}%
	\ifx\CF@current@arrowtype\@empty\def\CF@current@arrowtype{->}\fi
	\@testopt{\CF@arrow@iii(#1.#2[#3]--#4.#5[#6])}{}%
}

\CF@def\CF@arrow@iii(#1.#2[#3]--#4.#5[#6])[#7]{%
	\def\CF@tmp@str{\CF@arrow@v(#1.#2[#3]--#4.#5[#6])}%
	\CF@arrow@iv#7,\@empty,\@empty\@nil
}

\CF@def\CF@arrow@iv#1,#2,#3\@nil{%
	\CF@add@tocs\CF@tmp@str{{#1}}%
	\CF@expadd@tocs\CF@tmp@str{\expandafter{#2}}%
	\expandafter\CF@expadd@tocs\expandafter\CF@tmp@str\expandafter{\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#3,\@empty\@nil}}%
	\CF@tmp@str
}

% #1, #4 : nom des nodes    #2, #5 : ancres des nodes    #3, #6 : stryles des nodes
% #7 : angle fl\`eche    #8 : longueur fl\`eche    #9 : style tikz de la fl\`eche
\CF@def\CF@arrow@v(#1.#2[#3]--#4.#5[#6])#7#8#9{%
	\let\CF@arrow@current@style\CF@arrow@style
	\if\string @\expandafter\@car\detokenize{#1.}\@nil% "." au cas o\`u #1 est vide
		\if\string @\expandafter\@car\detokenize{#4.}\@nil
			\CF@expadd@tocs\CF@direct@arrow@list{\expandafter\CF@direct@arrow\expandafter{\CF@current@arrowtype}{#1}{#2}{#4}{#5}{#9}}%
			\let\CF@next@action\CF@schemestart@iii
		\else
			\unless\ifx\CF@arrow@current@style\@empty\CF@add@tocs\CF@arrow@current@style,\fi
			\ifx\@empty#9\@empty\else\CF@add@tocs\CF@arrow@current@style{#9,}\fi
			\CF@display@compound{}{#3}%
			\def\CF@next@nodename{#4}%
			\expandafter\def\expandafter\CF@current@nodename\expandafter{\@gobble#1}%
			\let\CF@arrow@start@name\CF@current@nodename
			\let\CF@arrow@end@name\CF@next@nodename
			\CF@arrow@vi{#7}{#8}{#2}{#5}%
			\def\CF@next@nodestyle{#6}%
		\fi
	\else
		\unless\ifx\CF@arrow@current@style\@empty\CF@add@tocs\CF@arrow@current@style,\fi
		\ifx\@empty#9\@empty\else\CF@add@tocs\CF@arrow@current@style{#9,}\fi
		\if\string @\expandafter\@car\detokenize{#2.}\@nil
			\errmessage{Package \CF@package@name\space Error: syntax "(<name>--@<name>)" is not allowed}%
		\else
			\CF@display@compound{#1}{#3}%
			\edef\CF@arrow@start@name{\ifx\@empty#1\@empty\CF@current@nodename\else#1\fi\ifx\@empty#2\@empty\else.#2\fi}%
			\CF@arrow@vi{#7}{#8}{#2}{#5}%
			\def\CF@next@nodename{#4}%
			\def\CF@next@nodestyle{#6}%
		\fi
	\fi
	\CF@arrow@gobspaces% mange les espaces puis ex\'ecute \CF@next@action
}

\CF@def\CF@arrow@gobspaces{\futurelet\CF@toks@a\CF@arrow@gobspaces@i}

\CF@def\CF@arrow@gobspaces@i{%
	\ifx\@sptoken\CF@toks@a
		\expandafter\CF@arrow@gobspaces@ii
	\else
		\expandafter\CF@next@action
	\fi
}

{\def\:{\CF@arrow@gobspaces@ii}\expandafter}\expandafter
\def\: {\futurelet\CF@toks@a\CF@arrow@gobspaces@i}

\CF@def\CF@arrow@vi#1#2#3#4{% #1=angle   #2=longueur    #3=ancre d\'epart   #4=ancre arriv\'ee
	\def\CF@next@action{\let\CF@compound\@empty\CF@schemestart@iii}%
	\def\CF@arrow@current@angle{#1}\ifx\@empty\CF@arrow@current@angle\let\CF@arrow@current@angle\CF@arrow@angle\fi
	\def\CF@current@arrow@length{#2}\ifx\@empty\CF@current@arrow@length\let\CF@current@arrow@length\CF@arrow@length\fi
	\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep),cyan,fill](end@arrow@i){};%
	\edef\CF@arrow@end@name{end@arrow@i\ifx\@empty#4\@empty\else.4\fi}%
	\ifCF@reac@debug
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@arrow@offset),red,fill](start@arrow){};%
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep-\CF@arrow@offset),red,fill](end@arrow){};%
	\else
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@arrow@offset)](start@arrow){};%
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep-\CF@arrow@offset)](end@arrow){};%
	\fi
	\def\CF@arrow@start@node{start@arrow}\def\CF@arrow@end@node{end@arrow}%
	\csname\expandafter\CF@grab@arrow@name\CF@current@arrowtype[\@nil\expandafter\expandafter\expandafter\endcsname
		\expandafter\CF@grab@arrow@args\CF@current@arrowtype[]\@nil[][][][][][][][]\@nil
	\def\CF@current@nodename{end@arrow@i}%
	\edef\CF@next@nodeanchor{\ifx\@empty#4\@empty180+\CF@arrow@current@angle\else#4\fi}%
}

% trace un fl\`eche initi\'ee par (@nom--@nom)
% #1=type de fl\`eche   #2=nom depart   #3=ancre d\'epart    #4=nom arriv\'ee    #5=ancre arriv\'ee    #6=style fl\`eche
\CF@def\CF@direct@arrow#1#2#3#4#5#6{%
	\path[sloped,allow upside down](\@gobble#2\ifx\@empty#3\@empty\else.#3\fi)--(\@gobble#4\ifx\@empty#5\@empty\else.#5\fi)%
		coordinate[pos=0,xshift=\CF@arrow@offset](start@direct@arrow)%
		coordinate[pos=1,xshift=-\CF@arrow@offset](end@direct@arrow);%
	\def\CF@arrow@start@node{start@direct@arrow}%
	\def\CF@arrow@end@node{end@direct@arrow}%
	\expandafter\def\expandafter\CF@arrow@start@name\expandafter{\@gobble#2}%
	\expandafter\def\expandafter\CF@arrow@end@name\expandafter{\@gobble#4}%
	\def\CF@arrow@current@style{#6}%
	\csname\CF@grab@arrow@name#1[]\@nil\expandafter\endcsname\CF@grab@arrow@args#1[]\@nil[][][][][][][][]\@nil
}

\CF@def\CF@merge@grab@chardir#1[#2][#3]#4\@nil{%
	\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@car#1>\@nil\@nil
	\ifx>\CF@toks@a\def\CF@merge@angle{0}\def\CF@merge@extreme{xmax}\def\CF@merge@sign{+}\else
	\ifx<\CF@toks@a\def\CF@merge@angle{180}\def\CF@merge@extreme{xmin}\def\CF@merge@sign{-}\else
	\ifx^\CF@toks@a\def\CF@merge@angle{90}\def\CF@merge@extreme{ymax}\def\CF@merge@sign{+}\else
	\ifx v\CF@toks@a\def\CF@merge@angle{-90}\def\CF@merge@extreme{ymin}\def\CF@merge@sign{-}%
	\fi\fi\fi\fi
	\def\CF@merge@labelup{#2}\def\CF@merge@labeldo{#3}%
}

\CF@def\merge#1({%
	\CF@merge@grab@chardir#1[][]\@nil
	\CF@merge@i(}

\CF@def\CF@merge@i#1--(#2){\@testopt{\CF@merge@ii#1--(#2)}{}}

\CF@def\CF@merge@ii#1--(#2)[#3]{%
	\CF@display@compound{}{}%
	\CF@parse@mergeopt#3,\@empty,\@empty,\@empty\@nil
	\def\CF@merge@xmax{-16383.99999pt}\let\CF@merge@ymax\CF@merge@xmax
	\def\CF@merge@xmin{16383.99999pt}\let\CF@merge@ymin\CF@merge@xmin
	\CF@merge@parse@nodelist#1(\relax)% calcule les maxi des positions
	\pgfmathparse{\csname CF@merge@\CF@merge@extreme\endcsname\CF@merge@sign\CF@merge@fromcoeff*\CF@compound@sep}%
	\let\CF@merge@extreme@result\pgfmathresult
	\CF@merge@iii#1(\relax)% trace les lignes entre les noeuds pr\'ec\'edents et la ligne de jonction
	\expandafter\def\expandafter\CF@tmp@str\expandafter{\expandafter[\CF@merge@style,shorten <=0,shorten >=0]}%
	\if x\expandafter\@car\CF@merge@extreme\@nil
		\CF@add@tocs\CF@tmp@str{(\CF@merge@extreme@result pt,\CF@merge@ymax)--(\CF@merge@extreme@result pt,\CF@merge@ymin)}%
	\else
		\CF@add@tocs\CF@tmp@str{(\CF@merge@xmin,\CF@merge@extreme@result pt)--(\CF@merge@xmax,\CF@merge@extreme@result pt)}%
	\fi
	\expandafter\draw\CF@tmp@str node[pos=\CF@merge@splitcoeff](merge@point){}% trace la ligne de jonction
		node[at=(merge@point),shift=(\CF@merge@angle:\CF@compound@sep*\CF@merge@tocoeff-\CF@arrow@offset)](end@merge){}%
		node[at=(merge@point),shift=(\CF@merge@angle:\CF@compound@sep*\CF@merge@tocoeff)](end@merge@i){};%
	\let\CF@arrow@current@angle\CF@merge@angle
	\expandafter\draw\expandafter[\CF@merge@style,shorten <=0,-CF@full](merge@point)--(end@merge)%
		\expandafter\CF@arrow@display@label@i\expandafter{\CF@merge@labelup}{.5}+\expandafter\CF@arrow@display@label@i\expandafter{\CF@merge@labeldo}{.5}-;%
	\def\CF@current@nodename{end@merge@i}%
	\let\CF@tmp@str\@empty
	\CF@analyse@arrowarg{#2}%
	\expandafter\CF@merge@iv\CF@tmp@str\@nil
}

\CF@def\CF@merge@iii(#1){%
	\if\relax\expandafter\noexpand\@car#1\@nil
	\else
		\CF@if@stop{#1}%
			{\edef\merge@current@nodename{\CF@before@stop#1\@nil}\edef\merge@current@anchor{\CF@after@stop#1\@nil}}%
			{\def\merge@current@nodename{#1}\let\merge@current@anchor\CF@merge@angle}%
		\if x\expandafter\@car\CF@merge@extreme\@nil
			\pgfextracty\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
			\expandafter\draw\expandafter[\CF@merge@style,shorten >=0]([shift=(\CF@merge@angle:\CF@arrow@offset)]\merge@current@nodename.\merge@current@anchor)--(\CF@merge@extreme@result pt,\CF@dim);%
		\else
			\pgfextractx\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
			\expandafter\draw\expandafter[\CF@merge@style,shorten >=0]([shift=(\CF@merge@angle:\CF@arrow@offset)]\merge@current@nodename.\merge@current@anchor)--(\CF@dim,\CF@merge@extreme@result pt);%
		\fi
		\expandafter\CF@merge@iii
	\fi
}

\CF@def\CF@merge@iv#1.#2[#3]\@nil{%
	\def\CF@next@nodename{#1}%
	\edef\CF@next@nodeanchor{\ifx\@empty#2\@empty180+\CF@merge@angle\else#2\fi}%
	\def\CF@next@nodestyle{#3}%
	\let\CF@compound\@empty
	\CF@schemestart@iii
}

\CF@def\CF@parse@mergeopt#1,#2,#3,#4\@nil{%
	\def\CF@merge@fromcoeff{#1}\ifx\@empty\CF@merge@fromcoeff\def\CF@merge@fromcoeff{0.5}\fi
	\expandafter\def\expandafter\CF@merge@tocoeff\expandafter{#2}\ifx\@empty\CF@merge@tocoeff\def\CF@merge@tocoeff{0.5}\fi
	\expandafter\def\expandafter\CF@merge@splitcoeff\expandafter{#3}\ifx\@empty\CF@merge@splitcoeff\def\CF@merge@splitcoeff{0.5}\fi
	\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@merge@style\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#4,\@empty\@nil}%
}

\CF@def\CF@merge@parse@nodelist(#1){%
	\if\relax\expandafter\noexpand\@car#1\@nil
	\else
		\CF@if@stop{#1}%
			{\edef\merge@current@nodename{\CF@before@stop#1\@nil}\edef\merge@current@anchor{\CF@after@stop#1\@nil}}%
			{\def\merge@current@nodename{#1}\let\merge@current@anchor\CF@merge@angle}%
		\pgfextractx\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
		\ifdim\CF@dim>\CF@merge@xmax\edef\CF@merge@xmax{\the\CF@dim}\fi
		\ifdim\CF@dim<\CF@merge@xmin\edef\CF@merge@xmin{\the\CF@dim}\fi
		\pgfextracty\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
		\ifdim\CF@dim>\CF@merge@ymax\edef\CF@merge@ymax{\the\CF@dim}\fi
		\ifdim\CF@dim<\CF@merge@ymin\edef\CF@merge@ymin{\the\CF@dim}\fi
		\expandafter\CF@merge@parse@nodelist
	\fi
}

\CF@def\CF@grab@arrow@name#1[#2\@nil{#1}
\CF@def\CF@grab@arrow@args#1[#2\@nil{[#2}

\CF@def\CF@make@parameter@text#1{%
	\toks\z@{}%
	\CF@cnt@groupnumber#1\relax
	\CF@make@parameter@text@i1%
}

\CF@def\CF@make@parameter@text@i#1{%
	\unless\ifnum#1>\CF@cnt@groupnumber
		\toks\z@\expandafter{\the\toks\z@[###1]}%
		\expandafter\CF@make@parameter@text@i\expandafter{\number\numexpr#1+1\expandafter}%
	\fi
}

% #1 est le nombre d'arguments optionnels, #2 est le nom et #3 le code
\CF@def\definearrow#1#2#3{%
	\begingroup
		\CF@make@parameter@text{#1}%
	\expandafter\endgroup
	\expandafter\def\csname\detokenize{#2}\expandafter\endcsname\the\toks\z@{#3\CF@gobble@tonil}%
}

\CF@def\CF@if@stop#1{\CF@if@stop@i#1.\@nil}
\CF@def\CF@if@stop@i#1.#2\@nil{\ifx\@empty#2\@empty\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}
\CF@def\CF@before@stop#1.#2\@nil{#1}
\CF@def\CF@after@stop#1.#2\@nil{#2}

\CF@def\CF@rotate@node*#1#2\@nil{\CF@if@stop{#1}{\CF@before@stop#1\@nil}{#1}}
\CF@def\CF@anchor@node*#1#2\@nil#3{\CF@if@stop{#1}{\CF@after@stop#1\@nil}{\CF@arrow@current@angle-#390-#1}}

% #1 = label  #2 = position  #3 = + ou - (au dessus ou au dessous)  #4 : nom du noeud de d\'epart
% #5 = label  #6 = position  #7 = + ou - (au dessus ou au dessous)  #8 : nom du noeud de fin
\CF@def\CF@arrow@display@label#1#2#3#4#5#6#7#8{%
	\ifx\@empty#1#5\@empty\else
		\path(#4)--(#8)\CF@arrow@display@label@i{#1}{#2}{#3}\CF@arrow@display@label@i{#5}{#6}{#7};%
	\fi
}

\CF@def\CF@arrow@display@label@i#1#2#3{%
	\ifx\@empty#1\@empty\else
		\if*\expandafter\@car\detokenize{#1}\@nil
			\ifCF@reac@debug
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep,draw,fill,cyan](shifted@node){}%
				node[draw,rotate=\CF@rotate@node#1\@nil,anchor=\CF@anchor@node#1\@nil#3,at=(shifted@node)]{\expandafter\@gobble\@gobble#1}%
			\else
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep](shifted@node){}%
				node[rotate=\CF@rotate@node#1\@nil,anchor=\CF@anchor@node#1\@nil#3,at=(shifted@node)]{\expandafter\@gobble\@gobble#1}%
			\fi
		\else
			\ifCF@reac@debug
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep,draw,fill,cyan](shifted@node){}%
				node[draw,pos=#2,anchor=-#390,sloped,yshift=#3\CF@arrow@labelsep]{#1}%
			\else
				node[pos=#2,anchor=-#390,sloped,yshift=#3\CF@arrow@labelsep]{#1}%
			\fi
		\fi
	\fi
}

% pose des noeuds d\'ecal\'es de la dimension #1 \`a (\CF@arrow@start@node) et (\CF@arrow@end@node)
\CF@def\CF@arrow@shift@nodes#1{%
	\unless\ifdim\ifx\@empty#1\@empty\z@\else#1\fi=\z@
		\edef\CF@tmp@str{%
			\noexpand\path(\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=#1](\CF@arrow@start@node1){}node[pos=1,sloped,yshift=#1](\CF@arrow@end@node1){};}%
		\CF@tmp@str
		\edef\CF@arrow@start@node{\CF@arrow@start@node1}\edef\CF@arrow@end@node{\CF@arrow@end@node1}%
	\fi
}

\definearrow3{->}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<-}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@full-](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow5{-/>}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node)%
		coordinate[midway,shift=(\CF@arrow@current@angle:-1pt)](midway@i)%
		coordinate[midway,shift=(\CF@arrow@current@angle:1pt)](midway@ii)%
		coordinate[at=(midway@i),shift=(\ifx\@empty#4\@empty225\else#4+180\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@start)%
		coordinate[at=(midway@i),shift=(\ifx\@empty#4\@empty45\else#4\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@end)%
		coordinate[at=(midway@ii),shift=(\ifx\@empty#4\@empty225\else#4+180\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@start@i)%
		coordinate[at=(midway@ii),shift=(\ifx\@empty#4\@empty45\else#4\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@end@i);
	\draw(line@start)--(line@end);%
	\draw(line@start@i)--(line@end@i);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<->}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@full-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<=>}{%
	\CF@arrow@shift@nodes{#3}%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=1,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=1,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node%
}

\definearrow3{<->>}{%
	\CF@arrow@shift@nodes{#3}%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0.2,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=1,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=0.8,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node%
}

\definearrow3{<<->}{%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0.2,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=0.8,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=1,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow30{%
	\CF@arrow@shift@nodes{#3}%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node}

\definearrow5{-U>}{% #4=coeff du rayon de l'arc de cercle  #5=1/2 angle
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node)node[midway](Uarrow@arctangent){};%
	\edef\CF@tmp@str{\ifx\@empty#1\@empty[draw=none]\fi}%
	\expandafter\draw\CF@tmp@str (Uarrow@arctangent)%
		arc[radius=\CF@compound@sep*\CF@current@arrow@length*\ifx\@empty#4\@empty0.333\else#4\fi,start angle=\CF@arrow@current@angle-90,%
		delta angle=-\ifx\@empty#5\@empty60\else#5\fi]node(Uarrow@start){};
	\edef\CF@tmp@str{[\ifx\@empty#2\@empty draw=none,\fi-CF@full]}%
	\expandafter\draw\CF@tmp@str (Uarrow@arctangent)%
		arc[radius=\CF@compound@sep*\CF@current@arrow@length*\ifx\@empty#4\@empty0.333\else#4\fi,start angle=\CF@arrow@current@angle-90,%
		delta angle=\ifx\@empty#5\@empty60\else#5\fi]node(Uarrow@end){};
	\edef\CF@tmp@str{\if\string-\expandafter\@car\detokenize{#4.}\@nil-\else+\fi}%
	\CF@arrow@display@label{#1}{0}\CF@tmp@str{Uarrow@start}{#2}{1}\CF@tmp@str{Uarrow@end}%
}

\pgfarrowsdeclare{CF@half}{CF@half}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfarrowsleftextend{-\CF@arrow@size}\pgfarrowsrightextend{.5\pgflinewidth}}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfsetdash{}\z@\pgfsetroundjoin\pgfsetroundcap
	\pgfpathmoveto{\pgfpoint\z@\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint{-.5\CF@arrow@size}\z@}%
	\pgfpathlineto{\pgfpoint\z@\z@}%
	\pgfusepathqfillstroke}

\pgfarrowsdeclare{CF@full}{CF@full}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfarrowsleftextend{-\CF@arrow@size}\pgfarrowsrightextend{.5\pgflinewidth}}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfsetdash{}\z@\pgfsetroundjoin\pgfsetroundcap
	\pgfpathmoveto{\pgfpoint\z@\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint{-.5\CF@arrow@size}\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{-.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint\z@\z@}%
	\pgfusepathqfillstroke}

\CF@savedcatcode

\endinput

######################################################################
#                             Historique                             #
######################################################################

v0.1        2010/06/23
	- Premi\`ere version publique sur le CTAN
----------------------------------------------------------------------
v0.2        2010/08/31
	- Ajout de la documentation en anglais.
	- Correction de bugs.
	- \printatom est d\'esormais une macro publique.
	- Les espaces sont permis dans les mol\'ecules. Ils seront
	  ignor\'es par d\'efaut puisque les atomes sont compos\'es en
	  mode math par \printatom
	- Une paire de Lewis peut \^etre repr\'esent\'ee ":".
	- Dans les cycles, une correction de la longueur du trait
	  d\'eport\'e des liaisons doubles est fait de telle sorte que si
	  l'on \'ecrit \chemfig{*5(=====)}, on obtient deux polygones
	  r\'eguliers concentriques.
	- La s\'equence de contr\^ole \setnodestyle permet de sp\'ecifier
	  le style des nœuds dessin\'es par tikz.
----------------------------------------------------------------------
v0.3        2010/11/21
	- Am\'elioration de \definesubmol qui accepte les s\'equences de
	  contr\^ole. On peut aussi choisir un alias dont la substitution
	  est diff\'erente selon l'orientation de la liaison qui lui
	  arrive dessus.
	- Le caract\`ere "|" force la fin d'un atome. Si on \'ecrit
	  "D|ef" alors, chemfig verra deux atomes "D" et "ef".
	- Le caract\`ere "#" est reconnu lorsqu'il suit un caract\`ere de
	  liaison. Il doit \^etre suivi d'un argument entre parenth\`eses
	  qui contient l'offset de d\'ebut et de fin qui s'appliqueront
	  \`a cette liaison.
	- La macro \chemfig admet un argument optionnel qui sera pass\'e
	  \`a l'environnement tikzpicture dans lequel elle est dessin\'ee
	- Mise en place de la repr\'esentation des m\'ecanismes
	  r\'eactionnels avec la synatxe "@{<nom>}" devant un atome o\`u
	  "@{<nom>,<coeff>}" au tout d\'ebut de l'argument d'une liaison.
	  Cette syntaxe permet de placer un nœud (au sens de tikz) qui
	  deviendra l'extr\'emit\'e des fl\`eches des m\'ecanismes.
	  Le trac\'e des fl\`eches est faite par la macro \chemmove dont
	  l'argument optionnel devient celui de l'environnement
	  tikspicture dans lequel sont faites les fl\`eches.
	- Pour le m\'ecanisme d'alignement vertical via le \vphantom, la
	  commande \chemskipalign permet d'ignorer le groupe d'atomes
	  dans lequel elle est \'ecrite.
	- La commande \chemname permet d'afficher un nom sous une
	  mol\'ecule. la commande \chemnameinit initialise la plus grande
	  profondeur rencontr\'ee.
	- La commande \lewis a \'et\'e modifi\'ee de telle sorte que les
	  dessins des d\'ecorations soient proportionnels \`a la taille
	  de la police.
----------------------------------------------------------------------
v0.3a       2011/01/08
	- Correction d'un bug dans l'argument optionnel de \definesubmol
	  lorsque celui-ci comporte des crochets.
	- Mise \`a jour du manuel en anglais.
	- Ajout de \vflipnext et \hflipnext pour retourner
	  horizontalement ou verticalement la prochaine mol\'ecule.
----------------------------------------------------------------------
v0.4        2011/03/07
	- chemfig est d\'esormais \'ecrit en plain-etex et donc
	  utilisable par d'autres formats que LaTeX.
	- Un peu plus de rigueur avec les catcodes des caract\`eres
	  sp\'eciaux, notamment lorsque la commande \chemfig se trouve
	  dans l'argument de \chemmove, \chemabove, \chembelow, \chemrel.
	  TODO : faut-il \scantoker l'argument de \chemfig pour \^etre
	  d\'efinitivement d\'ebarass\'e de ces histoires de catcode ???
	- Correction d'un bug dans le calcul de l'angle des liaisons
----------------------------------------------------------------------
v0.4a       2011/04/10
	- Correction d'un bug concernant l'argument optionnel en d\'ebut
	  de mol\'ecule.
----------------------------------------------------------------------
v0.4b       2011/04/24
	- l'argument de \chemfig est tok\'enis\'e avec \scantokens ce qui
	  rend caduc tout souci de code de cat\'egorie, \`a part #.
	- la commande \setbondstyle permet de d\'efinir le style des
	  liaisons.
	- correction de l'affichage incorrect des doubles liaisons dans
	  les cycles apr\`es les commandes \hflipnext et \vflipnext
	- correction d'un bug lorsqu'un alias commence une mol\'ecule
----------------------------------------------------------------------
v1.0       2011/06/15
	- les sch\'emas r\'eactionnels sont d\'esormais disponibles.
	- \Chemabove et \Chembelow modifient la boite englobante.
	- \Lewis modifie la boite englobante
	- les macros \chemleft, \chemright, \chemup et \chemdown
	  affichent des d\'elimiteurs extensibles \`a gauche, \`a droite,
	  au dessus et au dessous d'un mat\'eriel.
----------------------------------------------------------------------
v1.0a      2011/09/18
	- les macros \Lewis et \lewis admettent un argument optionnel
	- la macro \setlewisdist r\`egle la distance entre les 2 \'electrons

==> t-chemfig.tex <==
%  __________________________________________________________________
% |                                                                  |
% |                                                                  |
% |                           chemfig v1.0a                          |
% |                                                                  |
% |                        September 18, 2011                        |
% |                                                                  |
% |__________________________________________________________________|
%
% This is t-chemfig.tex, the package file for conTeXt.
%
% Maintainer: Christian Tellechea
% E-mail    : unbonpetit@gmail.com
%             Comments, bug reports and suggestions are welcome.
% Licence   : Released under the LaTeX Project Public License v1.3c or
%             later, see http://www.latex-project.org/lppl.txt
% Copyright : Christian Tellechea 2010-2011
%
% The "chemfig" package consists of the 8 following files:
%   chemfig.tex (the code of the package)
%   chemfig.sty (the package file for LaTeX)
%   t-chemfig.tex (this file)
%   README
%   chemfig_doc_en.tex, chemfig_doc_en.pdf (english manual)
%   chemfig_doc_fr.tex, chemfig_doc_fr.pdf (manual in french)
%
% --------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
% %     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% --------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% --------------------------------------------------------------------
\usemodule[tikz]%
\input chemfig.tex
\endinput
